Large Deviation Theory for Bose Gas of Photons and Planck's Oscillators

We utilize large deviation theorems to analyze the distributions of a Bose gas of photons and Planck's identical linear oscillators. By applying the Boltzmann-Sanov and Cram\'er-Chernoff theorems, we calculate the large deviation probabilities, entropies, and rate functions for the spatial and energy distributions of both photons and Planck's oscillators. Our study reproduces the results of Bose and Planck within the framework of large deviation theory.

==> Grammarly1.tex <==
Large Deviation Statistics for the Distributions of Open Systems, Ideal Linear Oscillators, Light Quanta, Ideal Gases, and Magnetic System
D. P. Shinde
168-A, Panchsheel Colony, Pachgaon, Kolhapur, State-Maharashtra, India - 416013.
dpshinde.physics@gmail.com

We apply the large deviations theorems of Boltzmann-Sanov and Cramer-Chernoff, respectively, to the distributions of the spatial arrangements and the total number of particles and total internal energy of the open systems. The entropies obtained from both theorems are negative of their respective large deviation rate functions. We have found that the inequality (equality) of the total entropy change of the grand ensemble for the irreversible (reversible) processes of the spatial arrangements of systems and energy-particle exchange with the reservoirs are analogous to that of the generalized second law of thermodynamics. We extend the applications of large deviation statistics for the macroscopic variables of systems of the ideal Planck's and Fermi's linear oscillators, light quanta, ideal gases, and particles with spin. By Lagrange's method of undetermined multipliers, the sets of the most probable or mean values of the members of a system are obtained for a statistical equilibrium.

The asymptotic methods are essential for the constructions of limit theorems, laws of large numbers, and various convergence criteria for the sums of random variables. Besides, in general, these topics are very useful to understand the relevance of the mathematical theory of probability in all branches of science. In statistical physics, the distributions of internal energies and numbers of systems, considered as macroscopic random variables, of an ensemble, under generalized conditions, follow the central limit theorem (CLT) or Laplace-Gauss law of probability. The normal deviations of internal energies and numbers of systems from their respective mean values considered by CLT are used for understanding the states of equilibrium of the systems and ensemble. The modern large deviation theory (LDT) in its simple mathematical form or abstract probability measure-theoretic form determines the asymptotic probabilities and their decay rates for the random variables in rare events. 
However, physicists did not utilize the combination of Boltzmann-Sanov and Cramer-Chernoff large deviations theorems for the distributions of spatial arrangements of systems and their internal energies. A comparative study of the large deviations for the macroscopic variables of the distinguishable and indistinguishable systems has not been done. On the other hand, mathematical studies on the large deviations consider neither specific physical models of an isolated ensemble and ensemble-heat reservoir, respectively, for the distributions of spatial arrangements and the total internal energy of closed systems nor the reversible and irreversible diffusion processes of matter and energy. Besides, clear and coherent physical interpretations or inferences on the connections of large deviation entropies or rate functions with the laws of thermodynamics, relative fluctuations in the entropies, and entropy productions in the thermodynamical processes have not been shown.

Following Lagrange's method of undetermined multipliers, the D-variations of entropies with respect to the numbers of systems (particles) of an ensemble (an ideal gas) for the state of statistical equilibrium should vanish subject to the restrictive conditions, 'S(1)-S(2)=0'. 
This statistical equilibrium condition provides the mean or most probable set of values for the numbers of systems (particles) of an ensemble (an ideal gas). The entropies 'S1' and 'S2' are proportional to their respective logarithms of the probability distributions. The entropy 'S(1)=k*logP1+constant' is obtained from the joint or multinomial spatial probability distribution 'P1' of the systems subject to some constraints on the macroscopic variables of the ensemble. But, following the restrictive conditions on the total numbers of systems 'N' and total internal energy 'E' of an ensemble, the entropy 'S(2)=A+B'is directly written in terms of Lagrange's undetermined multipliers 'A' and 'B'. The parameters 'A' and 'B'. are related, respectively, to the inverses of a partition function 'Z' and the absolute temperature 'T'. However, for the entropy 'S(2)', the form of probability distribution was unknown. 

The recent study on the large deviations for the probability distributions distributions 'P1' and 'P2' of the random variables of closed systems has shown that a correct combination of the Boltzmann-Sanov and Cramer-Chernoff theorems provide the statistical equilibrium condition via Lagrange's method of undetermined multipliers. It shows clear and coherent interpretations of the large deviations results for the distributions of spatial arrangements and the internal energies of the closed systems. In particular, the spatial distribution of the systems 'P1' is obtained at a constant total energy of the closed and isolated ensemble whereas the distribution 'P2' is defined as probability inequality for the total internal energy of the ensemble at the constant total number of systems. Moreover, it has been shown that the large deviations results on the entropies or rate functions are connected in terms of equalities and inequalities, analogous to the laws of thermodynamics,  with the other thermodynamical variables in both reversible and irreversible diffusion processes of matter and energy. It is clearly stated that the large deviation rate functions are identical either to Boltzmann's 'H' or to Gibbs 'E' function. Furthermore, in the case of the coupled model of the ensemble and the heat reservoir, the physical significance of the large deviations results for the study of the relative fluctuations in the entropies is also illustrated.

%The modern large deviation theory (LDT) calculates the asymptotic probabilities of independent and dependent random variables beyond their normal deviations, exponential decay rates of probabilities, and determines the various mathematical properties of the rate functions. However, previous studies on the large deviations for the physical systems ignore the correct combination of Boltzmann-Sanov and Cramer-Chernoff theorems for determining the statistical equilibrium condition for the distributions of numbers of systems and their internal energies.  In particular, in the statistical equilibrium condition, Lagrange's undetermined parameters A and B are directly written from the restrictive conditions on the total number of systems and total internal energy of the ensemble. These parameters appear naturally by following the Cramer-Chernoff bound on the probability inequality for the total internal energy of the ensemble. Besides, the clear, continuous, and coherent physical interpretations on the connections of large deviation entropies or rate functions with the laws of thermodynamics have not been shown. Particularly, the logical connections of large deviations entropies or rate functions in terms of equalities and inequalities with other thermodynamical variables or functions are completely missing in previous studies. Furthermore, the use of large deviation theory for the relative fluctuations of entropies in case of coupling of ensemble and heat reservoir, and entropy productions in the irreversible diffusion processes of matter and energy are not studied. Mathematical studies on the large deviations consider neither specific physical models of an isolated ensemble and ensemble-heat reservoir for the distributions of spatial arrangements and the total internal energy of closed systems nor the reversible and irreversible diffusion processes of matter and energy. Most importantly, the physical interpretations or meanings of the known results on the large deviations and their various terms are not clearly stated in previous mathematical studies. 

%However, for the determination of the statistical equilibrium condition, previous studies on the large deviations for the physical systems ignore the correct combination of Boltzmann-Sanov and Cramer-Chernoff theorems, respectively, for the distributions of spatial arrangements of systems and their internal energies. Besides, the clear, continuous, and coherent physical interpretations on the connections of large deviation entropies or rate functions with the laws of thermodynamics have not been shown. In particular, the logical connections of large deviations entropies or rate functions in terms of equalities and inequalities with other thermodynamical variables or functions in the reversible and irreversible processes are completely missing in the previous studies. Furthermore, the use of large deviation theory for the relative fluctuations of entropies for the coupled of ensemble and heat reservoir, and for the entropy productions in the irreversible diffusion processes of matter and energy are not studied. Mathematical studies on the large deviations consider neither specific physical models of an isolated ensemble and ensemble-heat reservoir for the distributions of spatial arrangements and the total internal energy of closed systems nor the reversible and irreversible diffusion processes of matter and energy. Moreover, the physical significance or meaning of the known results on the large deviations is not stated for the information about states of physical systems. 

An ensemble is an imaginary collection of a large number of identical copies of a system that has a resemblance with the actual physical system. Three major types of ensembles, micro-canonical, canonical, and grand canonical are useful to study the thermodynamical properties of the classical and quantum physical systems. For these ensembles, various macroscopic variables and the state functions are defined for an individual system and the whole ensemble in their respective state spaces. For the given macro-states, the systems of the three ensembles have similar sets of values of their respective macroscopic variables. The sum of macroscopic variables of the systems defines a macroscopic variable for a certain macro-state of the whole ensemble. In equilibrium statistical mechanics, the ensemble averaging technique i.e. the averaging of a macroscopic variable over a large number of systems of an ensemble is equivalent to the time averaging technique for the same macroscopic variable. The systems of the micro-canonical ensemble are closed and isolated from the surroundings whereas the closed systems of canonical ensemble exchange only energy to the heat reservoir. 
The grand canonical ensemble consists of open systems which exchange both energy and particles with the heat and particle reservoirs respectively. To obtain the probability distribution of an unspecified open system, Gibbs defined a probability-coefficient 'Pg' and the index of probability 'N= *log*P(g)' as a function of macroscopic variables, the total internal energy, and the total number of particles of the grand canonical ensemble. Following Gibbs, for the grand canonical ensemble, we have 'P(g)=e^(O-E*T)', and 'N=log*P(g)= (O-E)/T', where 'T=1/kT' ('k' is Boltzmann constant and 'T' is absolute temperature), and 'M's are chemical potential of the components of the grand canonical ensemble. 

The large deviations of the general open systems and other various classical and quantum systems have not been studied. We plan our large deviation study on these systems as follows.
In the general case, we study the large deviations for the random variables, the numbers, and internal energies, of the large numbers of open classical systems of the grand canonical ensemble. In particular, we apply, respectively, the Boltzmann-Sanov theorem, for the joint spatial distributions of open systems of an isolated ensemble and the Cramer-Chernoff theorem for the distribution of the total internal energy and the total number of particles of the ensemble that couples to the heat and particle reservoirs. Moreover, in both cases, we obtain the entropy and rate functions for the macro-state of the ensemble. Furthermore, we suggest inequality (equality), analogous to the generalized second law of thermodynamics, of total entropy change of the grand ensemble in irreversible (reversible) processes of spatial arrangements of open systems and energy-particle exchange to the reservoirs. The thorough large deviation analysis gives the entropies and rate functions for the distributions of the spatial arrangements and energies of Planck's and Fermi's ideal linear oscillators, light quanta, particles of the ideal gases, and the particles with spins. For all these case studies, we obtain the statistical equilibrium conditions using the method of Lagrange undetermined multipliers. 

%In equilibrium statistical mechanics, the ensemble averaging technique i.e. the averaging of a macroscopic variable over a large number of systems of the ensemble is equivalent to the time averaging technique for the same macroscopic variable. Moreover, these ensemble theories are applicable to study the statistics of the macroscopic variables of systems of ideal linear oscillators, light quanta, classical and quantum ideal gases, and particles with spins. In the statistical equilibrium, the distributions of macroscopic variables such as internal energies and numbers of the systems of particles in the systems, under the generalized conditions, asymptotically follow the Laplace-Gauss or normal probability law. The deviations from the respective mean values of macroscopic variables, following the normal law, are called the normal deviations. To obtain the joint spatial distribution of the various open systems and distribution of the total internal energy and the total number of particles of the ensemble, respectively, the ensemble is isolated from its surroundings and is attached to the heat and particle reservoirs.
 
%This article, following the Boltzmann-Sanov theorem, provides large deviations for the joint spatial distribution of open systems, and the entropy and rate functions for the macro-state of the grand canonical ensemble. Besides, we use Cramer-Chernoff's theorem for calculations of the large deviation upper bound on the probability, the entropy, and the rate functions for the total internal energy and the total number of particles of the ensemble. The thorough large deviation analysis gives the entropies and rate functions for the distributions of the spatial arrangements and energies of Planck's and Fermi's ideal linear oscillators, light quanta, particles of the ideal gases, and the particles with spins. For all these case studies, we obtain the statistical equilibrium conditions using the method of Lagrange undetermined multipliers. 

{General Case: Large Deviations for Open Systems} 
%In the general case, we study the large deviations of the random variables, the numbers and internal energies, of the open classical systems of the grand canonical ensemble. In particular, we apply, respectively, the Boltzmann-Sanov theorem, for the joint spatial distributions of open systems of an isolated ensemble and Cramer-Chernoff theorem for the distribution of the total internal energy and the total number of particles of the ensemble which couple with the heat and particle reservoirs. The grand canonical ensemble consists of very large number X of macroscopic, quasi-independent, distinguishable or indistinguishable open systems.
{Joint or Multinomial Spatial Distribution: For Quasi-Independent Distinguishable Systems}

First, we construct a joint or multinomial spatial distribution of a very large number 'X(t)' of macroscopic, quasi-independent, and distinguishable systems at a given set of values of (T, V, m), where V is the volume and then repeating the same procedure, write down large deviations results for the quasi-independent and indistinguishable systems. 

At any given instant of time, let 'X(i, N)' be the number of systems having the number of particles 'N'  and energy 'E(i)' in the states of an 'i-th' partition. The subscripts 'i' and 'N' denote, respectively, an 'i-th' partition of the phase-space of the whole ensemble and the number of particles in a system. The energy 'E(i)' of the system in the given macro-state varies with the number of particles. The macroscopic variables 'X(i, N)', 'N', and 'E(i)', regarded as random variables, of the states, fluctuate about their respective mean values. The probability of finding an unspecified open system of a grand ensemble in a particular macro-state depends on a certain amount of energy and the number of particles of that macro-state. This is also defined as a ratio of the number of systems 'X(i, N)' that lies in the states an 'i'-th partition to the total number of systems 'X(t)'. Let 'W(N)' denotes a probability of finding a single system in any one of the states of an 'i'-th partition with the energy 'E(i)' and the number of particles 'N'. Then, the occupation probability of 'X(i, N)' systems in the states of an 'i'-th partition is
'W,(N)X(i,N)'. The macroscopic configuration '(X(i, N);i=1,...,r)' of spatial arrangements of all systems over the states of all the partitions, following some restrictive conditions, can be realized in a number of ways. This is also known as the joint or multinomial spatial distribution of all the systems subject to restrictive conditions. The three restrictive conditions fix the total number of systems 'X(t)', total internal energy 'E(t)', and the total number of particles 'N(t)' of the ensemble. 
These restrictive conditions are defined in the following way
(i)N*X(i,N)= X(t), (ii)N*E(i)X(i,N)=X(t)E*=E(t), i(ii),N*N(i)*X(i,N)=X(t)N* =N(t),
where 'X(i,N)> 0', 'E(i)> 0', 'N(i)> 0'. The ratios 'E*=E(t)/X(t)' and 'N*=N(t)/X(t)', respectively, the mean energy and mean number of the particles per system remain constants in the infinite limits of 'E(t)', 'N(t)', and 'X(t)'. The sum in equation2 is the double sum and it runs over 'i' and 'N'. The use of combinatorics, satisfying the equation 2, provides the final form of the joint spatial distribution 'P(b)' of the quasi-independent and distinguishable systems 
'P(b)(X(i,N);i=1,...,)= X!*[W(N)^X(i,N)/X(i,N)!]', 
where '0 < W(N) < 1' and 'W(N)=1'. 
Now first, we take the natural logarithm on both sides of equation 2 and then use Stirling's approximation for the factorials of large numbers 'X! ~ X*log*X-X' and 'X(i,N)! ~ X(i,N) *log*X(i,N) -X(i,N)'. Thus, we get the equations
'log*P(b)(.)=log*X ! + [X(i,N)*log*W(N)-log*X(i,N)!]',
'log*P(b)(.)=log*X ! + [X(i,N)*log*W(N)-log*X(i,N)!]'.
The total Boltzmann-Sanov entropy 'S(b)' of the ensemble is proportional to the logarithm of the probability function 'log*P(b)'. Therefore, from the lower line of equation 3, we have the expression for the entropy 'S(b) = k*log*P(b)', where k is the Boltzmann constant. Dividing on both sides of the lower line of equation 3 by 'X', we have,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'X*log*P(b)(.) ~ F(i,N)*log*(W(N)/F(i,N))',
where 'F(i,N) =X(i,N)/X' is the ratio of the number of systems that fall in the 'i-th' partition to the total number of systems, and 'F(i,N)=1'. The thermodynamic limit 'X to infinity for 'X/*log*P(b)(.)' exists and from the lower line of equation 4, the function 'S(b)=F(i,N)*log*(W(N)/F(i,N))' is the Boltzmann-Sanov entropy of a single system. In addition, it is a sum of cross entropy and the entropy of mixing. In this case of joint spatial distribution, the Boltzmann-Sanov rate function for a single system is negative of its entropy (negentropy) function, 'I(b)=-S(b)=F(i,N)*log(F(i,N)/W(N)) = [F(i,N)*W(N)*log*(F(i,N)/W(N))]'. 

Entropy, probability function, and information are linked to each other. The rate function 'I(F, W)' is also known as Kullback-Leibler (K-L) divergence or discrimination information between 'F' and 'W'. If 'W' refers to the relative volume of a partition and approximates F then I(F, W) (negentropy) is the information loss about the system's state. A principle of the maximum of entropy is equivalent to the principle of a minimum of the K-L divergence. Here, the Gibbs inequality is written as ' -F(i,N)* log* F(i,N) <  -F(i,N)*log*W(i,N). The forms of entropy and rate functions for the ensemble are as follows, 'S(1b) =X*S(b)' and 'I(1b) =X*I^(b)'. Here both 'I(b)' and 'I(1b)' are non-negative (> 0).
 
%{For Quasi-Independent and Indistinguishable Systems}

For the quasi-independent and indistinguishable systems, we use the correct form of a joint spatial probability distribution and repeat the procedure from equations  2 to 4. The joint spatial distribution 'P(b)' and its natural logarithm, entropy, and rate functions are given below
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))= S(b)/k',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=- I^(b)'.

% Cramer-Chernoff Upper Bound for Total Internal Energy and Total Number of Particles
%Quasi-Independent and Distinguishable Systems

Now, let us consider the distribution of the macroscopic random variables of the state, the total internal energy 'E(t)' and the total number of particles 'N(t)'. The ensemble exchanges energy to a heat reservoir of temperature 'T' and particles to the particle reservoir of the chemical potential 'M'. 
To obtain the large deviation bound, the generalized form of the Bienayme-Chebyshev-Markov (BCM) probability inequality is used.  This generalized probability inequality expresses in terms of the moment generating function (MGF) or partition function and given thresholds of the random variables.
For the given random variables 'E(t)' and 'N(t)' of the ensemble, we define a new non-negative, real-valued exponential variable 'e^(-B(E(t)-M N(t))' with two real-valued parameters 'B' ('=1/kT') and the chemical potential 'M'. 
In the case of quasi-independent and distinguishable systems, Cramer and Chernoff large deviation upper bound 'P*(c)'  on the probability of 'e^(-B(E(t)-M N(t))' expresses in terms of the grand canonical partition function and the given thresholds on the energies and number of particles in the systems,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where 'B > 0', 'Z(B, M)' and 'Z(g)=(Z(B, M))^(X(t))' are the grand canonical partition functions of a single system and the ensemble respectively.
The symbol 'E' in the upper line of equation 6 denotes the mathematical expectation. 
The natural logarithm on both sides of 6, and then division on both sides by 'X(t)', supply
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.  
In equation 9, the limit X(t) to infinity exists. We know that the grand canonical entropy is proportional to the natural logarithm of the probability function 'P*(c)'. 
Equations 7 and 8 give the grand canonical entropies of the ensemble and single distinguishable system respectively, 'S*(c)=k*log*P*(c)=X(t)*[B*E- B*MN + log*Z(B,M)]' and 'S(E, N) =S*(c)/X(t) = k*[B*E+A*N + log*Z(B, A)]', where 'A = -B*M'. The Cramer-Chernoff  large deviation rate function for a single distinguishable system is 'I(E, N) =[-B*E-A*N- log*Z(B, A)] = [(B*G-E)- A*N] ', where the function 'G(B,A)=-(B^(-1))*log*Z(B,A)' is the Gibbs free energy. The rate function 'I(E, N)' shows duality with the Massieu potential function or Planck's characteristic function 'P(B,A)' '(= -B*G =log*Z(B,A)' through the Legendre-Fenchel transform 'log*Z(B, A) =[-B*E-A*N- I(E, N)]'. The rate function the grand canonical ensemble is written as 'I(N)= X(t)*I(E, N)'. We observe that the The Cramer-Chernoff large deviation rate function 'I(c)' or 'I1(E, N)' is identical to the Gibbs index of probability 'N'.  


%Quasi-Independent and Indistinguishable Systems
In the case of quasi-independent and indistinguishable systems, we put the correct form of the grand canonical partition function of the ensemble 'e^(-B*E(t)-M*N(t))/X(t)!' into equation 6 and then follow the steps of calculations of equations 7, and 8. In this case, the Crammer-Chernoff upper bound 'P*(c)' and its natural logarithm, and grand canonical entropy and rate functions are written as
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.
From equation 10, we get the total grand canonical entropy of the ensemble 'S*(c)= k*log*P*(c) = X(t)*S(1c),', where 'S(E, N)=k*[B*E+A*N +log*(eZ/X(t))]' is the entropy of a single indistinguishable system. The Cramer-Chernoff large deviation function for a single indistinguishable system is 'I(E, N)=-k*[B*E+A*N +log*(eZ/X(t))]'.  

%Statistical Equilibrium Condition for the Open Systems
The method of Lagrange's undetermined multipliers subject to restrictive conditions gives the most probable set of the systems 'X(i, N)' for each 'i' at the statistical equilibrium. The entropy or the logarithmic probability function attains the maximum value at the statistical equilibrium. In equations 4 and 8, the entropies $ 'S(b)' and S*(c) are functions of 'X(i,N)'. At the statistical equilibrium, the differentials of logarithmic functions 'dP(b)' and 'dP*(c)', or equivalently the differentials of entropies 'dS(b)' and 'dS*(c)', subject to the variations of the three constraints X=0, Y=0, and Z=0, vanish. 
Following the method of Lagrange's undetermined multipliers, we equate the total variations 'd' of equations 3 and 7 with respect to 'X(i, N)' to zero 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.
where, 'e^(B*G)=1/Z' ,. For the equal values of 'W(N)', we get the probability of finding a distinguishable system in a state with energy 'E(i)' and number of particles 'N(i)', 'X(i,N)/X(t) = e^(- B*E(i)-M*N(i))/Z(B,A)'. By utilizing the total variations of equations 5 and 10, we can obtain a similar expression as that of equation 12, for the probability of finding an indistinguishable system. However, the differences in the Boltzmann-Sanov and grand canonical entropies for indistinguishable and distinguishable cases are functions of 'X(t)'. 

The substitution of 'X(i, N)' from equation 13 into three constraints equation 2 furnishes the expressions for the grand partition function, mean energy, and mean number of particles per system respectively 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.
Using the expressions of 'E*' and 'N*' from 13 in equation 7, the mean grand-canonical entropy per system 'S(c) = S*(c)/X(t)', is,
'S(c) =k[B*E+A*N+ log*Z^(g)]', 
'X=kk[B*E+A*N+ log*Z^(g)]'. 
The recent study of the large deviations shows the connections of entropies or rate function, in terms of equalities and inequalities, with other thermodynamical variables in the reversible and irreversible processes.  
For the reversible processes, the differential of the total Boltzmann-Sanov entropy 'S(b)' shows equality with the differentials of Gibbs free energy and the mean work-done and inequality for the irreversible spatial arrangements of the systems. On the other hand, in the reversible process of the energy and particle with the reservoirs, the differential of total grand canonical entropy establishes equality with differentials of total mean internal energy, total work, and total mean number of particles, 'dS*(c)=B*dQ(c)= B*[dE*(c)+dW(c)-M*dN(c)]'. Both processes of spatial arrangements of the systems and the exchange process of the energy and particle with the reservoirs produce entropy. The entropy productions are zero (always positive) in the reversible (irreversible) processes of spatial arrangements of the open systems and energy and particle exchange with the respective reservoirs. The change in the total entropy of the grand ensemble occurs either due to the production of entropy in the spatial arrangements of open systems inside the ensemble or entropy exchange to or from the heat and particle reservoir. These assertions establish equalities (inequalities) of the total entropy production in the reversible (irreversible) processes of the spatial arrangements and energy-particle exchange 'dS(j)= dS(b)+dS(c)>0'. The upper line of equation 16 shows a strong similarity with the generalized form of the second law of thermodynamics that developed for the black-hole entropy. The middle and lower lines are the equalities (inequalities) of the entropy productions in the reversible (irreversible) diffusion processes that occur interior and exterior of the grand canonical ensemble.

%\sectionLarge Deviations for Spatial and Energy Distributions of Various Systems
Here, we study the large deviations for the distributions of macroscopic variables of various systems such as Planck's and Fermi's ideal linear oscillators, classical and quantum ideal gases, and the magnetic system of particles with spin. Previous studies on these systems utilized the Boltzmann's distribution for the spatial arrangements of members of a system and determined the most probable values using Lagrange's method of undetermined multipliers subject to the restrictive conditions on the total numbers of members and total energy of the system. Moreover, these studies ignored the BCM type probability inequality either for the total internal energy or for both the total number of particles and the total internal energy of the whole ensemble. 

To obtain large deviation results for each of the systems mentioned here, we repeat the following steps: (1) Follow the restrictive conditions and construct the joint spatial distribution for the members of a system and then, by taking the natural logarithm of spatial distribution and using Stirling's approximation for the factorials, obtain Boltzmann-Sanov entropy and rate functions for the macro-state a system and its member. (2) Calculate first the Cramer-Chernoff large deviation probability upper bound either on the total energy or both total numbers of members and the total energy of a system and then use of the natural logarithm of probability function and Stirling's approximation for the factorials provide the entropy and rate functions for the macro-state a system and its member. (3) Establish the statistical equilibrium condition from the differentials of either Boltzmann-Sanov and canonical or grand canonical entropies or the large deviation rate functions by using Lagrange's method of undetermined multipliers and by following the total variation of restrictive conditions on the total energy and total numbers of members of a system. 

% up to here.
%Planck Case: System of the Ideal Linear Oscillators
Planck considered a distribution of the ideal linear oscillators over the infinitesimal region elements of the state-space of the whole system. The notations are similar to those of Planck's book and his research articles. Let '(N=N1+N2+...+N(n)+...)' and '(E=E1+E2+...+E(n)+...)' be the total number of oscillators and the total energy of a system respectively. The subscript 'n' denotes the labeled region elements '(1,2,...,n,....)' of the state-space of a system. The variables 'N(n)' and 'E(n)' are the number of oscillators and their energies in the 'n-th' region respectively. The energy 'E(n)' of the 'N(n)' oscillators with the equal frequency 'f' in the 'n-th' region is 'E(n)=N(n)*(n-1/2)*h*f =  N*w(n)*(n-1/2)h*f', where 'h' is Planck's constant and 'w = Nn/N' is a distribution density. Here, the term '(n-1/2)*h*f' is the arithmetic mean of energies '(n-1)*h*f' and 'n*h*f' of the oscillators in the 'n-th' region. One can also take arithmetic mean over 'n' and 'n+1' region elements; then energy becomes 'E(n)=N(n)*(n+1/2)*h*f'. Moreover, the total energy 'E' of the whole system is the sum of energies of oscillators in all region elements  'E = N*h*f *(n-1/2)*w(n)', where 'w(n) = N(n)/N' is a probability. We can rewrite the total energy as 'E = N*U*', where 'U* = (n-1/2)*w(n)*h*f' is the mean energy per oscillator. 

Following step (1) and the constraints on the total number and total energy of the oscillators, we write large deviations results for the joint spatial distribution of the 'N' quasi-independent linear oscillators over all the region elements
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where 'N(n) > 0', 'w(n)=N(n)/N', '0< w(n)<1', and 'w(n)=1'. From equation 16, the total Boltzmann-Sanov entropy of the system is  'S(bp) = k*log*P(bp) ~ k*[N(n)*log*N - N(n)*log*N(n)]'. Besides, equation 18 gives the entropy of a single ideal oscillator is the mean logarithm of 'w(n)', 'S(bp)= S(bp)/N = -k*[w(n)*log*w(n)]=-k*(<log*w(n)>)'. The Boltzmann-Sanov rate functions for the system and single oscillator are negative of their respective entropies.

Step (2) gives the Cramer-Chernoff large deviation upper bound for the exponential variable of the total energy 'E' of the system. 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
Here 'B>0' and the symbol 'E' in equation 18 denotes the mathematical expectation, and 'Z1(B)=e^(-B*E1)' and 'Z(B)=e^(-B*E)=(e^(-B^E1))^(N)' are the partition functions, respectively, of the single oscillator and the whole system. The equations 19 and 20 supply the expressions, respectively, for the total canonical entropy of the system and the canonical entropy per oscillator 'S*(cp)=k*log*P*(cp) = k *[B*N*U+ N*log*Z1] ' and 'S(cp) = S*(cp)/N=k*[B*N*U+ N*log*Z1]'. For the system and an oscillator, the Cramer-Chernoff large deviation rate functions are 'I=-S/k' and 'I1=S1/k'.

At the statistical equilibrium, the 'd' variations of the entropies with respect to 'N(n)' vanish i.e. 'dS(bp) =0' and 'dS*(cp) =0'. We follow step (3) and get the statistical equilibrium condition for the most probable set of Planck's linear oscillators,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
where the partition function of an oscillator, 'Z1(B)=e^(-B*(n-1/2)*h*N)', is obtained by putting 21 in the condition 'N=N(n)'. Therefore, from equation 21, 'w(n)=e^(-B*(n-1/2)*h*N)' is the probability of finding exactly 'N(n)' oscillators in the 'n-th' region element. To obtain equation 21, we can also consider 'd' variations of equations 17 and 20 with respect to 'w(n)' and follow Lagrange's method of undetermined multipliers.
Using equation 21, the mean energy, 'U*' and mean entropy per oscillator 'S(cp)'  are written, respectively, as
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 

Planck defined a large positive number, the integer 'R' that measures the energy of the system of oscillators, 'R= (E/h*f) -(N/2)=(n-1)*N(n)'. Therefore, by step (1), for a given energy of the system, the joint spatial distribution of 'N' oscillators or the total number of distinct ways of assigning 'R' quanta to 'N' oscillators is
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
Follow step (2) and the Cramer-Chernoff upper bound of the total energy of the system of oscillators is  
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where we have put 'N*U=Rh*ft. The term 'Z1(B)' is the partition function of a single oscillator. Planck replaced the total energy 'E= N*U' of a system of 'N' oscillators with the discrete energy packets of large positive number 'R' (quanta) with finite equal quantity 'h*N', i.e. X=Y/N. Thus, 'E/N=U/N', where 'hu/2' is the zero-point energy.
By considering step (3), for the statistical equilibrium condition, the variations 'dR' of both sides of equations 24 and 26 vanish. 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
The mean energy per oscillator 'E/N' 
E(n)/N=(X*R*N+X)*h*N.

%Bose Case: System of Light Quanta
Let us consider Bose's famous work on the statistics of light quanta. Bose obtained the probability distribution of the light quanta that lie into the various cells of the phase-space of the whole system. Moreover, he reproduced Planck's results of the total entropy of the thermodynamic state and total energy density of the system of the light quanta. We apply steps (1) to (3) sequentially and obtain the large deviations for the distributions of the number of the light quanta and their energies.  The chemical potential 'm' is zero for a system of the light quanta. Here, we follow similar notations found in Bose's work.

Let 'As=Ps,r' be the total number of labeled cells '(Ps0,Ps1,....,P(s,r),...)' in the 's-th' infinitesimal frequency interval 'df'. The index 'r' indicates the number of light quanta in the cells of 'df' . The total number of light quanta and their total energy in the cells of 'df' are 'N(s)=P(s,r)' and 'E(s)=Ps*r*h*fs'  respectively.  These quantities per cell are written as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'
where 'w(r) =Ps,r/As' is a probability, and 'b*' and 'U*(sb)' are, respectively, the mean number of light quanta and their mean energy per cell of 'df'.
Step (1) provides the results for the joint distribution of the cells containing the various number of light quanta in 'df'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
The mean energy per oscillator 'E/N' 
E(n)/N=(X*R*N+X)*h*N.
The distribution over all infinitesimal frequency intervals is the product of distributions, 'P(bb)=W(bb)'. From, 31 and 32, we write the total Boltzmann-Sanov entropy 'S(bb)', and entropy per cell 'S(bb)/As' respectively.
'S(bb) = k *log*W(bb) ~ k *log*(As/P(s,r))', 
S(bb) = k *log*W(bb) ~ k *log*(As/P(s,r))'. 
Moreover, the total entropy of the system over all infinitesimal frequency intervals is 'S(bb) =S(bb)'. The Boltzmann-Sanov rate function are 'I(bb) =-S(bb)' and 'I1(bb) =-S1(bb)'
Considering step (2), for 'B>0, we have expressions for the Cramer-Chernoff large deviation upper bound on the probability of the total energy 'E(s)' of the light quanta, the natural logarithm of probability function, the canonical entropy and Cramer-Chernoff rate function in the interval 'df'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where '(Z(1,b))^(As)' is the partition function over all 'As' cells. The chemical potential 'M' is zero for the system of the light quanta. The distribution over all infinitesimal frequency intervals is 'P*(c)b=W(bb)'  
Equations 34 and 36 provide the expressions for the total canonical entropy 'S(sb)' and entropy per cell 'S(sb)/As' respectively.
'S(cb)= k *log*W(cb) = [k*B*r*fs + k*r*log*Z(1,b)]', 
'S(cb)= k *log*W(cb) = [k*B*r*fs + k*r*log*Z(1,b)]'. 
Following step (3), the equilibrium condition  is obtained by equating the deviations 'd' on both sides of equations 31 and 35 either with respect to 'ps,r' or with respect to 'w(s,r)' to zero. Here we equate 'dP(s,r)' to zero,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
where the partition function 'Z(1,b)(B)= e^(-B*r*h*fs)= (1-e^(-B*h*fs))^(-1)' is obtained from the condition 'r=0*P(s,r)= As'. The lower line of equation 38 gives the probability of exactly 'r' number of light quanta that lie in the cells of the interval 'df'. 
Using equation 38, the mean number of light quanta per cell in 'df'  is 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
This is identical with Planck's result (See equation 28).
Moreover, 'N*b=bs= e^(B*h*fs -1)' is the total mean occupancy number of the system of light quanta. 
Using equation 38, the total energy 'E(s)' and energy of the light quanta  per cell in 'df' are obtained, respectively, as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The energy of the whole system of light quanta over all the frequency intervals is 'E(b)=E(s)=B(s)', . 
The mean Gibbs canonical entropy in 'df' at the equilibrium ,is, 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
where in the second line of equation 41, we have put 'U*(sb)' from equation 40 and logarithm of 'Z(1,b)'. Moreover, the mean Gibbs canonical entropy per cell ,in 'df' from the last line of equation 41 is 
X*S(cb)*As = X*B*h*fs*e^(-B*h*fs-1*log*(1- e^(-B*h*fs)).
Equation 43 is identical to equation 23.
The entropy of the whole system of light quanta over all the frequency intervals is 'S(cb) =M*S(cb)'. 

%Fermi Case: System of Simple Oscillators
Schroedinger studied a simple system of the Fermi oscillators with zero chemical potential. Here the notations are identical to those of Bose's case. The Pauli exclusion principle restricts the number of oscillators (particles) per cell i.e. either  'r=0' or 'r=1' in each cell. The restrictive conditions are defined on the total number of cells 'As', total number of Fermi oscillators 'N(f)' and their energies 'E(f)' in the 's-th' interval, 'As = p(s)', 'N(s)=r*p(s)' and 'E(s)=r*e*p(s)', where 'e' is the energy of a single Fermi oscillator.

Step (1) gives us the joint spatial distribution 'W(bf)' of cells that filled with the oscillators, the total Boltzmann-Sanov entropy 'S(bf)' of the system, and entropy per cell 'S(bf)/As'. 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.'
The last line of equation 44 can be rewritten as 'k*log*W/A=S/A=k<log(w)> '.
We have the total spatial distribution for all the intervals 'P(bf)= W(bf)' and 'S(bf)=S(bf)'.
We consider step (2) and obtain the Cramer-Chernoff's large deviation bound, logarithmic probability function, canonical entropy for the total energy distribution of system of Fermi's oscillators 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
where 'B>0' and 'Z(1,f)=e^(-r*B*E)= (1+e^(-B*E))' is the partition function of a single Fermi oscillator respectively. For the whole system and all the intervals, we get 'P*(cf)=W(cf)' and 'S(cf)= S(cf)'. 
The use of step (3) provides the equilibrium condition for a system of the Fermi oscillators i.e. the most probable values of the oscillators. Equate the 'd' variations of the second line of equation 43 and the third line of equation 44 to zero.  
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
The lower line of equation 45 defines the probability of finding the Fermi oscillator in the cells of the 's' interval. Using this definition of the probability, equation 47, the mean occupation number of the oscillators per cell 'Sf' is given as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The total occupancy number is 'N*(f)=e^(B*E+1)'. 
Using equation 47, the total energy 'ESf' of oscillators and mean energy per cell and mean energy per cell 'U(sf)f' in the 's-th' interval are written as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'. 
Putting equation 47 in the mean entropy of oscillators and the mean entropy of oscillators per cell in the 's-th' interval, we get 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The total entropy of the system of the Fermi oscillators is 'Sf =N*S(cf)'.  

%Classical and Quantum Ideal Gases
In the previous sections, we have considered the systems of Planck and Fermi ideal linear oscillators, and light quanta with zero chemical potential. Here, we focus on the large deviations study for the distributions of the non-relativistic classical and quantum ideal gases with nonzero chemical potentials. The particles of the ideal gases obey three different types of statistics: (i) Maxwell-Boltzmann (MB) (ii) Bose-Einstein (BE), and (iii) Fermi-Dirac (FD). 
Due to weak interactions between the particles, they are assumed quasi-independent, and thus, the probabilities of macroscopic variables of the particles do not affect each other. Thus the problem of studying the statistics of macroscopic variables of the whole ideal gas reduces to that of studying the statistics of a single particle. Particles of the MB ideal gas are distinguishable and have no restrictions on occupancy in a single state. Bose-Einstein (BE) statistics allows any number of identical and indistinguishable particles (bosons) with integer spin in a single state. In the Fermi-Dirac ideal gas, a single state can not accommodate simultaneously more than one identical and indistinguishable particle (fermion) with half-integral spin because of the restriction of the Pauli exclusion principle. 
Quantum mechanically, the solution for the statistics of an ideal gas is to find the number of symmetric (antisymmetric) eigenfunctions for a boson (fermion) state. Let 'G(j)', 'N(j)', and 'E(j)' be the number of states, number of particles, and their energies in the 'j'-th group. The aggregate of the number of particles '(N(j), j=1,2,...)' into the states of the independent labeled groups 'j=1,2,...' defines the macroscopic state of the whole ideal gas. The total number of particles and total energy of the ideal gas are written as 'N(j)= Nt' and 'N(j)*E(j) = Et'. 

Our first aim is to find the distribution of the 'N(j)' particles that lie into the 'G(j)' states in the 'j'-th group and then in succession construct a distribution for all the independent groups of states. This is equivalent to finding the statistical weight i.e. the number of distinct ways 'G(j)' of distributing 'N(j)' particles over a state in the 'j-th' group. The total statistical weight for all the independent groups of the identical particles is the product of 'G(j)', i.e 'Pb(ig)^(G(j))'.  

Following step (1), the total statistical weights or joint spatial distributions of the particles of the three different types of ideal gases, satisfying the constraints on the total numbers of particles and total energy of the ideal gas, are written as  
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The total entropy of an ideal gas is proportional to the natural logarithm of the total statistical weight i.e. 'S(g) ~ k*log*P(ig)= k**log*G(j)'. 
'S(g) ~ k*log*P(ig)= k**log*G(j)',
'S(g) ~ k*log*P(ig)= k**log*G(j)',  
'S(g) ~ k*log*P(ig)= k**log*G(j)'.  
The use of step (2) gives us the Cramer-Chernoff large deviation upper bound on the probability of the variable 'e^(-B*E(t)-M*N(t))', the grand canonical entropy, and the Cramer-Chernoff rate function. 
'P*(c)< e^(-B*E(t)-M*N(t))',
'P*(c)< e^(-B*E(t)-M*N(t))', 
'P*(c)< e^(-B*E(t)-M*N(t))'.
where 'Zg(B,M)' is a grand partition function of whole ideal gas 
and 'A= -B*M'.  We put 'N(t) =N(j)' and 'N(t)U = N(j) E(j) ', and the logarithms of the grand partition functions for the MB, BE, and FD ideal gases in equation 53.
'log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',
'log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'.
We know that the grand canonical entropy for a macroscopic state of an ideal gas is proportional to the natural logarithm of a probability distribution, 'S*(ig) ~k*log*P*(ig); thus, 'S*(ig)= k*log*P*(ig) = S(ig)'. 
Consider step (3), the variations 'dN(j)' on both sides of the set of equations 51 and 54 provide the statistical equilibrium conditions for the set of most probable or mean values of the particles in the three different types of ideal gases.
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',  
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'. 
we get the mean occupation number of the particles in each of the state of 'j-th' group.
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',  
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'. 
The total mean occupancy number of the particles in an ideal gas is 'N=N*(j)'. 

%Magnetic System: Particles with Spins
The absolute temperature 'T' or the parameter 'B=1/kT' is nonnegative, i.e. 'T > 0' or 'B > 0', for for the closed or open normal thermodynamical system.  The internal energy of a normal system varies from zero (0) or a certain least attainable value, say E(+0) to the infinity ('I').
Here we follow steps (1) to (3) and study the large deviations for the distributions of numbers of particles and the total energy of a magnetic system. The internal energy of a magnetic system has both the lower 'Em,+0' and upper 'E-0' bounds, respectively,  for the temperatures 'T tends to +0' and 'T tends to -0'. 

Consider a magnetic system of 'N' weakly interacting quasi-independent particles with a spin '1/2'. This magnetic system is placed in the external magnetic field 'H'; thus, each of the particles has two orientations with a magnetic moment either '+M' parallel to or '-M' antiparallel to the field 'H'. Moreover, the corresponding non-degenerate energies are '+e=+u*H' and  '-e=-u*H'. 
The total number of particles 'N' and the total internal energy 'E' of a system are written as 'N=N++N-' and 'E=(N+-N-)M*H = M*E' respectively, where 'N+' and 'N-' are, respectively, the '+' spin and '-' spin particles, and 'M=N+-N-' is the magnetization. The numbers N+' and 'N-' are expressed in terms of 'M' and 'E' as follows 'N+ = (N+M)/2 = (N*E+E)/2*E ' and 'N- = (N-M)/2 = (N*E-E)/2*E'.    

%For the cases of normal closed or open systems, the temperature 'T' or 'B=1/kT' is nonnegative i.e. 'T > 0' or 'B > 0'. The internal energy of the normal systems or an ensemble varies from '0' (or a certain least attainable value, say 'E+') to 'I'. For the positive attainable temperature 'T > ' or 'B > 0', the internal energy 'E' lie in the interval '(E0, E+] ', where 'E+'  is the maximum value for maximum temperature 'T to infinity ' or 'B tends to +0'. As the temperature 'T tends +0 ' or to least value, then the internal of a system shifts to 'E0', and entropy attains its minimum value. This is the case of the third law of thermodynamics.  The magnetic system of particles with spins is in completely different thermodynamical states for the positive 'T > 0' ('B > 0') and negative 'T < 0' ('B < 0') temperatures. Moreover, at these temperatures, the entropy of the system attains the minimum value but for two entirely different thermodynamics states. Here we study the large deviations for the distributions of the magnetic system corresponding to both positive and negative temperatures. Let 'N+' and 'N-' be, respectively, '+' spin and '-' spin particles. The total number of particles 'N' and the total energy 'E' of the system are written as 'N=N++N-' and 'E=(N+-N-)M H = ME', where 'M=N+-N-' and '*E=M H' respectively. Therefore, we have This system is always termed a 'two-level system'.

By step (1), the number of ways of the spatial arrangements of the N+' and 'N-'  particles in the energy states '+e' and '-e' the thermodynamic weight 'Pb' of a macroscopic state of a magnetic system takes the final form 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',  
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'. 

In the last line of Eq.58, 'w- = X*N/N' and 'w+=X*N/N' are the probabilities. The Boltzmann-Sanov type entropy ' S(mb)' is Boltzmann constant times the natural logarithm of '*log*P(mb)' i.e. 'S(mb)= k *log*P(mb)'. By putting the values of 'N-' and 'N+' in equation 58, we have the expressions for the total Boltzmann-Sanov type entropy of a system and entropy per particle
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N', 
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N'.

From equation 59, the temperature 'T' of the system is defined as '1/T = dS/dE=(k/*E)*log[(N*E-E)/(N*E+E)]' or '1/T=(k/*E)*log(N+/N-)'. This temperature is either positive or negative according to whether 'N*e < E' or 'N*e > E' 
The parameter 'T* =-1/T' covers the entire range of temperature from '+infinity' to '-infinity' including zero. Table 1 shows the values of 'T', internal energy 'E', and entropy 'S' of a system at various temperatures. The magnetic system is in a completely different thermodynamical states for the positive 'T > 0' ('B > 0') and negative 'T < 0' ('B < 0') temperatures. Moreover, at these temperatures, the entropy of a  system attains the minimum value, but for the entirely different thermodynamical states. In the case of positive temperature, the population in the higher energy state is small 'N(-) <N(+)', whereas for the negative temperature the population is large 'N(-) >N(+)'.
In the experiment on the LiF crystal, by reversing the magnetic field, the thermodynamic equilibrium with the population 'N(-) >N(+)' in the maximum energy state was achieved successfully for the negative temperature. 

We now calculate the Crammer Chernoff upper bound on the probability inequality of the total internal energy 'E' of a system that exceeds to certain threshold 'Nu', where u is the energy per particle. Since the magnetic system exhibits different behavior for both positive and temperature, therefore the maximums of the Crammer Chernoff rate functions are achieved for the intervals of positive and negative temperature with the corresponding ranges of the total internal energies. Therefore we need two probability inequalities for the two intervals of positive and negative temperature. In this case, the population, number of particles, in the maximum energy state is larger than the minimum energy state.

(i) For a  strictly positive temperature 'T >0' ('T* < 0') and corresponding range of the total internal energy of the system, 'Em,+0< E < N*u', we define the probability inequality of the total internal energy and the given threshold 'P*(c)+(E < N*u)=P*(c)+(-E > -N*u)=P*(c)+(-B*E > -B N*u)', where 'B > 0'. (ii)In the case of the negative temperature 'T < 0' ('T*> 0')  and respective range of the total internal energy of a system 'Nu < E < E-0', we get another probability inequality of the total internal energy and the given threshold, 'P*(c)-(E > N*u)=P*(c)-(-B*E > -B*N*u)', where 'B < 0'. Then in the both regimes of positive and negative temperatures of the magnetic system, following step (1), the Cramer-Chernoff large deviation upper bounds and their natural logarithms, canonical entropies and rate functions are written as
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N', 
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N'.
Here the partition function of the whole system is the product of partition functions of the quasi-independent weakly interacting particles. In addition, the Helmholtz free energy of the system is 'A= -N*k*T*log*Z1 = -N*k*T*log(2*cosh(B*E))'. 

Consider step (3) and obtain the statistical equilibrium condition by equating the variations 'd' on sides of the equations 59 and 61 with respect to 'N-' and 'N+'  to zero.
S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N', 
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N'.
The upper and lower lines of equation 62 define the probabilities of finding a single particle of the magnetic system, respectively, in the states 'E+ =M*H' and 'E-=-M*H'. 
The mean energies of a particle and the system are given as 'U* = -d*log(Z1)/dB = -*E*tanh(B*E)' and 'E= M*E= (N+-E-)*E = - N*E*tanh(B*E)=N*U' respectively. 
Moreover, the mean entropies of the system and per particle are, respectively, obtained as 'S(cm) = B*N*U*+N*log*Z(1) = N*k*[-B*E*tanh(B*E)+log(2*cosh(B*E)]' and 'S(mc)= S(cm)/N*k = -B*E*tanh(B*E+log(2*cosh(B*E))'.



%The thermodynamic states of the system at temperatures 'T tends to +_infinity ' are identical. For these temperatures, the internal energy reaches to the mean values 'E +_ infinity' and the entropy attains the maximums 'Sm,+_infinity= N*k*log2'.The parameter 'T* =-1/T' captures all ranges from positive to negative temperatures. 

%For the cases of closed or open normal thermodynamical systems, the temperature $T$ or $\beta=1/kT$ is nonnegative i.e. $T \geq 0$ or $\beta \geq 0$ \cite{LandauV5,Haar95,Schroedinger13,Pathria11,Greiner95}. The internal energy of the normal systems or an ensemble varies from $0$ (or a certain least attainable value, say $E_{+0}$) to $\infty$ \cite{LandauV5,Haar95,Schroedinger13,Pathria11,Greiner95}.  Here we study the large deviations for the distributions of the magnetic system corresponding to both positive and negative temperatures.  The magnetic system of particles with spins is in completely different thermodynamical states for the positive $T \geq 0$ ($\beta \geq 0$) and negative $T \leq 0$ ($\beta \leq 0$) temperatures \cite{Ramsey56,Purcell51}. The internal energy of a magnetic system has lower $\mathsf{E}_{min,+0}$ and upper $\mathsf{E}_{max,-0}$ bounds, respectively, as $T \to +0$ and $T \to -0$ \cite{Ramsey56,Purcell51}. Moreover, at these temperatures, the entropy of the system attains the minimum value but for two entirely different thermodynamics states \cite{Ramsey56,Purcell51}.


\sectionDiscussions and Summary

\bibliographyGrandRef

\enddocument
%
% ****** End of file apstemplate.tex ******



==> Grammarly2.tex <==
Large Deviation Statistics for the Distributions of Open Systems, Ideal Linear Oscillators, Light Quanta, Ideal Gases, and Magnetic System
D. P. Shinde
168-A, Panchsheel Colony, Pachgaon, Kolhapur, State-Maharashtra, India - 416013.
dpshinde.physics@gmail.com

We apply the large deviations theorems of Boltzmann-Sanov and Cramer-Chernoff, respectively, to the distributions of the spatial arrangements and the total number of particles and total internal energy of the open systems. The entropies obtained from both theorems are negative of their respective large deviation rate functions. We have found that the inequality (equality) of the total entropy change of the grand ensemble for the irreversible (reversible) processes of the spatial arrangements of systems and energy-particle exchange with the reservoirs are analogous to that of the generalized second law of thermodynamics. We extend the applications of large deviation statistics for the macroscopic variables of systems of the ideal Planck's and Fermi's linear oscillators, light quanta, ideal gases, and particles with spin. By Lagrange's method of undetermined multipliers, the sets of the most probable or mean values of the members of a system are obtained for a statistical equilibrium.


The asymptotic methods are essential for the constructions of limit theorems, laws of large numbers, and various convergence criteria for the sums of random variables. Besides, in general, these topics are very useful to understand the relevance of the mathematical theory of probability in all branches of science. In statistical physics, the distributions of internal energies and numbers of systems, considered as macroscopic random variables, of an ensemble, under generalized conditions, follow the central limit theorem (CLT) or Laplace-Gauss law of probability. The normal deviations of internal energies and numbers of systems from their respective mean values considered by CLT are used for understanding the states of equilibrium of the systems and ensemble. The modern large deviation theory (LDT) in its simple mathematical form or abstract probability measure-theoretic form determines the asymptotic probabilities and their decay rates for the random variables in rare events. 


However, the previous mathematical and physical studies on large deviations for distributions of the classical systems did not address the following points. 
I)A comparative study of large deviations for distinguishable and indistinguishable systems
ii)A formula for a probability occurrence of relative fluctuations in the Boltzmann-Sanov and Gibbs entropies for the non-isolated model of ensemble and heat-reservoir
iii)A connection between large deviation entropies or rate functions and the loss of heat or work or the Clausius uncompensated transformations ?
iv)A connection between large deviation entropies or rate functions to equality or inequality of the generalized second law of thermodynamics for the total entropy production, rather then ordinary form of second law of thermodynamics. 
V)The generalized De Donder type inequality for the entropy productions in the processes that occur interior and exterior of the ensemble



However, physicists did not utilize the combination of Boltzmann-Sanov and Cramer-Chernoff large deviations theorems for the distributions of spatial arrangements of systems and their internal energies. A comparative study of the large deviations for the macroscopic variables of the distinguishable and indistinguishable systems has not been done. On the other hand, mathematical studies on the large deviations consider neither specific physical models of an isolated ensemble and ensemble-heat reservoir, respectively, for the distributions of spatial arrangements and the total internal energy of closed systems nor the reversible and irreversible diffusion processes of matter and energy. Besides, clear and coherent physical interpretations or inferences on the connections of large deviation entropies or rate functions with the laws of thermodynamics, relative fluctuations in the entropies, and entropy productions in the thermodynamical processes have not been shown.

Following Lagrange's method of undetermined multipliers, the D-variations of entropies with respect to the numbers of systems (particles) of an ensemble (an ideal gas) for the state of statistical equilibrium should vanish subject to the restrictive conditions, 'S(1)-S(2)=0'. 
This statistical equilibrium condition provides the mean or most probable set of values for the numbers of systems (particles) of an ensemble (an ideal gas). The entropies 'S1' and 'S2' are proportional to their respective logarithms of the probability distributions. The entropy 'S(1)=k*logP1+constant' is obtained from the joint or multinomial spatial probability distribution 'P1' of the systems subject to some constraints on the macroscopic variables of the ensemble. But, following the restrictive conditions on the total numbers of systems 'N' and total internal energy 'E' of an ensemble, the entropy 'S(2)=A+B'is directly written in terms of Lagrange's undetermined multipliers 'A' and 'B'. The parameters 'A' and 'B'. are related, respectively, to the inverses of a partition function 'Z' and the absolute temperature 'T'. However, for the entropy 'S(2)', the form of probability distribution was unknown. 

The recent study on the large deviations for the probability distributions distributions 'P1' and 'P2' of the random variables of closed systems has shown that a correct combination of the Boltzmann-Sanov and Cramer-Chernoff theorems provide the statistical equilibrium condition via Lagrange's method of undetermined multipliers. It shows clear and coherent interpretations of the large deviations results for the distributions of spatial arrangements and the internal energies of the closed systems. In particular, the spatial distribution of the systems 'P1' is obtained at a constant total energy of the closed and isolated ensemble whereas the distribution 'P2' is defined as probability inequality for the total internal energy of the ensemble at the constant total number of systems. Moreover, it has been shown that the large deviations results on the entropies or rate functions are connected in terms of equalities and inequalities, analogous to the laws of thermodynamics,  with the other thermodynamical variables in both reversible and irreversible diffusion processes of matter and energy. It is clearly stated that the large deviation rate functions are identical either to Boltzmann's 'H' or to Gibbs 'E' function. Furthermore, in the case of the coupled model of the ensemble and the heat reservoir, the physical significance of the large deviations results for the study of the relative fluctuations in the entropies is also illustrated.

%The modern large deviation theory (LDT) calculates the asymptotic probabilities of independent and dependent random variables beyond their normal deviations, exponential decay rates of probabilities, and determines the various mathematical properties of the rate functions. However, previous studies on the large deviations for the physical systems ignore the correct combination of Boltzmann-Sanov and Cramer-Chernoff theorems for determining the statistical equilibrium condition for the distributions of numbers of systems and their internal energies.  In particular, in the statistical equilibrium condition, Lagrange's undetermined parameters A and B are directly written from the restrictive conditions on the total number of systems and total internal energy of the ensemble. These parameters appear naturally by following the Cramer-Chernoff bound on the probability inequality for the total internal energy of the ensemble. Besides, the clear, continuous, and coherent physical interpretations on the connections of large deviation entropies or rate functions with the laws of thermodynamics have not been shown. Particularly, the logical connections of large deviations entropies or rate functions in terms of equalities and inequalities with other thermodynamical variables or functions are completely missing in previous studies. Furthermore, the use of large deviation theory for the relative fluctuations of entropies in case of coupling of ensemble and heat reservoir, and entropy productions in the irreversible diffusion processes of matter and energy are not studied. Mathematical studies on the large deviations consider neither specific physical models of an isolated ensemble and ensemble-heat reservoir for the distributions of spatial arrangements and the total internal energy of closed systems nor the reversible and irreversible diffusion processes of matter and energy. Most importantly, the physical interpretations or meanings of the known results on the large deviations and their various terms are not clearly stated in previous mathematical studies. 

%However, for the determination of the statistical equilibrium condition, previous studies on the large deviations for the physical systems ignore the correct combination of Boltzmann-Sanov and Cramer-Chernoff theorems, respectively, for the distributions of spatial arrangements of systems and their internal energies. Besides, the clear, continuous, and coherent physical interpretations on the connections of large deviation entropies or rate functions with the laws of thermodynamics have not been shown. In particular, the logical connections of large deviations entropies or rate functions in terms of equalities and inequalities with other thermodynamical variables or functions in the reversible and irreversible processes are completely missing in the previous studies. Furthermore, the use of large deviation theory for the relative fluctuations of entropies for the coupled of ensemble and heat reservoir, and for the entropy productions in the irreversible diffusion processes of matter and energy are not studied. Mathematical studies on the large deviations consider neither specific physical models of an isolated ensemble and ensemble-heat reservoir for the distributions of spatial arrangements and the total internal energy of closed systems nor the reversible and irreversible diffusion processes of matter and energy. Moreover, the physical significance or meaning of the known results on the large deviations is not stated for the information about states of physical systems. 

An ensemble is an imaginary collection of a large number of identical copies of a system that has a resemblance with the actual physical system. Three major types of ensembles, micro-canonical, canonical, and grand canonical are useful to study the thermodynamical properties of the classical and quantum physical systems. For these ensembles, various macroscopic variables and the state functions are defined for an individual system and the whole ensemble in their respective state spaces. For the given macro-states, the systems of the three ensembles have similar sets of values of their respective macroscopic variables. The sum of macroscopic variables of the systems defines a macroscopic variable for a certain macro-state of the whole ensemble. In equilibrium statistical mechanics, the ensemble averaging technique i.e. the averaging of a macroscopic variable over a large number of systems of an ensemble is equivalent to the time averaging technique for the same macroscopic variable. The systems of the micro-canonical ensemble are closed and isolated from the surroundings whereas the closed systems of canonical ensemble exchange only energy to the heat reservoir. 
The grand canonical ensemble consists of open systems which exchange both energy and particles with the heat and particle reservoirs respectively. To obtain the probability distribution of an unspecified open system, Gibbs defined a probability-coefficient 'Pg' and the index of probability 'N= *log*P(g)' as a function of macroscopic variables, the total internal energy, and the total number of particles of the grand canonical ensemble. Following Gibbs, for the grand canonical ensemble, we have 'P(g)=e^(O-E*T)', and 'N=log*P(g)= (O-E)/T', where 'T=1/kT' ('k' is Boltzmann constant and 'T' is absolute temperature), and 'M's are chemical potential of the components of the grand canonical ensemble. 

The large deviations of the general open systems and other various classical and quantum systems have not been studied. We plan our large deviation study on these systems as follows.
In the general case, we study the large deviations for the random variables, the numbers, and internal energies, of the large numbers of open classical systems of the grand canonical ensemble. In particular, we apply, respectively, the Boltzmann-Sanov theorem, for the joint spatial distributions of open systems of an isolated ensemble and the Cramer-Chernoff theorem for the distribution of the total internal energy and the total number of particles of the ensemble that couples to the heat and particle reservoirs. Moreover, in both cases, we obtain the entropy and rate functions for the macro-state of the ensemble. Furthermore, we suggest inequality (equality), analogous to the generalized second law of thermodynamics, of total entropy change of the grand ensemble in irreversible (reversible) processes of spatial arrangements of open systems and energy-particle exchange to the reservoirs. The thorough large deviation analysis gives the entropies and rate functions for the distributions of the spatial arrangements and energies of Planck's and Fermi's ideal linear oscillators, light quanta, particles of the ideal gases, and the particles with spins. For all these case studies, we obtain the statistical equilibrium conditions using the method of Lagrange undetermined multipliers. 

%In equilibrium statistical mechanics, the ensemble averaging technique i.e. the averaging of a macroscopic variable over a large number of systems of the ensemble is equivalent to the time averaging technique for the same macroscopic variable. Moreover, these ensemble theories are applicable to study the statistics of the macroscopic variables of systems of ideal linear oscillators, light quanta, classical and quantum ideal gases, and particles with spins. In the statistical equilibrium, the distributions of macroscopic variables such as internal energies and numbers of the systems of particles in the systems, under the generalized conditions, asymptotically follow the Laplace-Gauss or normal probability law. The deviations from the respective mean values of macroscopic variables, following the normal law, are called the normal deviations. To obtain the joint spatial distribution of the various open systems and distribution of the total internal energy and the total number of particles of the ensemble, respectively, the ensemble is isolated from its surroundings and is attached to the heat and particle reservoirs.
 
%This article, following the Boltzmann-Sanov theorem, provides large deviations for the joint spatial distribution of open systems, and the entropy and rate functions for the macro-state of the grand canonical ensemble. Besides, we use Cramer-Chernoff's theorem for calculations of the large deviation upper bound on the probability, the entropy, and the rate functions for the total internal energy and the total number of particles of the ensemble. The thorough large deviation analysis gives the entropies and rate functions for the distributions of the spatial arrangements and energies of Planck's and Fermi's ideal linear oscillators, light quanta, particles of the ideal gases, and the particles with spins. For all these case studies, we obtain the statistical equilibrium conditions using the method of Lagrange undetermined multipliers. 

{General Case: Large Deviations for Open Systems} 
%In the general case, we study the large deviations of the random variables, the numbers and internal energies, of the open classical systems of the grand canonical ensemble. In particular, we apply, respectively, the Boltzmann-Sanov theorem, for the joint spatial distributions of open systems of an isolated ensemble and Cramer-Chernoff theorem for the distribution of the total internal energy and the total number of particles of the ensemble which couple with the heat and particle reservoirs. The grand canonical ensemble consists of very large number X of macroscopic, quasi-independent, distinguishable or indistinguishable open systems.
{Joint or Multinomial Spatial Distribution: For Quasi-Independent Distinguishable Systems}

First, we construct a joint or multinomial spatial distribution of a very large number 'X(t)' of macroscopic, quasi-independent, and distinguishable systems at a given set of values of (T, V, m), where V is the volume and then repeating the same procedure, write down large deviations results for the quasi-independent and indistinguishable systems. 

At any given instant of time, let 'X(i, N)' be the number of systems having the number of particles 'N'  and energy 'E(i)' in the states of an 'i-th' partition. The subscripts 'i' and 'N' denote, respectively, an 'i-th' partition of the phase-space of the whole ensemble and the number of particles in a system. The energy 'E(i)' of the system in the given macro-state varies with the number of particles. The macroscopic variables 'X(i, N)', 'N', and 'E(i)', regarded as random variables, of the states, fluctuate about their respective mean values. The probability of finding an unspecified open system of a grand ensemble in a particular macro-state depends on a certain amount of energy and the number of particles of that macro-state. This is also defined as a ratio of the number of systems 'X(i, N)' that lies in the states an 'i'-th partition to the total number of systems 'X(t)'. Let 'W(N)' denotes a probability of finding a single system in any one of the states of an 'i'-th partition with the energy 'E(i)' and the number of particles 'N'. Then, the occupation probability of 'X(i, N)' systems in the states of an 'i'-th partition is
'W,(N)X(i,N)'. The macroscopic configuration '(X(i, N);i=1,...,r)' of spatial arrangements of all systems over the states of all the partitions, following some restrictive conditions, can be realized in a number of ways. This is also known as the joint or multinomial spatial distribution of all the systems subject to restrictive conditions. The three restrictive conditions fix the total number of systems 'X(t)', total internal energy 'E(t)', and the total number of particles 'N(t)' of the ensemble. 
These restrictive conditions are defined in the following way
(i)N*X(i,N)= X(t), (ii)N*E(i)X(i,N)=X(t)E*=E(t), i(ii),N*N(i)*X(i,N)=X(t)N* =N(t),
where 'X(i,N)> 0', 'E(i)> 0', 'N(i)> 0'. The ratios 'E*=E(t)/X(t)' and 'N*=N(t)/X(t)', respectively, the mean energy and mean number of the particles per system remain constants in the infinite limits of 'E(t)', 'N(t)', and 'X(t)'. The sum in equation2 is the double sum and it runs over 'i' and 'N'. The use of combinatorics, satisfying the equation 2, provides the final form of the joint spatial distribution 'P(b)' of the quasi-independent and distinguishable systems 
'P(b)(X(i,N);i=1,...,)= X!*[W(N)^X(i,N)/X(i,N)!]', 
where '0 < W(N) < 1' and 'W(N)=1'. 
Now first, we take the natural logarithm on both sides of equation 2 and then use Stirling's approximation for the factorials of large numbers 'X! ~ X*log*X-X' and 'X(i,N)! ~ X(i,N) *log*X(i,N) -X(i,N)'. Thus, we get the equations
'log*P(b)(.)=log*X ! + [X(i,N)*log*W(N)-log*X(i,N)!]',
'log*P(b)(.)=log*X ! + [X(i,N)*log*W(N)-log*X(i,N)!]'.
The total Boltzmann-Sanov entropy 'S(b)' of the ensemble is proportional to the logarithm of the probability function 'log*P(b)'. Therefore, from the lower line of equation 3, we have the expression for the entropy 'S(b) = k*log*P(b)', where k is the Boltzmann constant. Dividing on both sides of the lower line of equation 3 by 'X', we have,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'X*log*P(b)(.) ~ F(i,N)*log*(W(N)/F(i,N))',
where 'F(i,N) =X(i,N)/X' is the ratio of the number of systems that fall in the 'i-th' partition to the total number of systems, and 'F(i,N)=1'. The thermodynamic limit 'X to infinity for 'X/*log*P(b)(.)' exists and from the lower line of equation 4, the function 'S(b)=F(i,N)*log*(W(N)/F(i,N))' is the Boltzmann-Sanov entropy of a single system. In addition, it is a sum of cross entropy and the entropy of mixing. In this case of joint spatial distribution, the Boltzmann-Sanov rate function for a single system is negative of its entropy (negentropy) function, 'I(b)=-S(b)=F(i,N)*log(F(i,N)/W(N)) = [F(i,N)*W(N)*log*(F(i,N)/W(N))]'. 

Entropy, probability function, and information are linked to each other. The rate function 'I(F, W)' is also known as Kullback-Leibler (K-L) divergence or discrimination information between 'F' and 'W'. If 'W' refers to the relative volume of a partition and approximates F then I(F, W) (negentropy) is the information loss about the system's state. A principle of the maximum of entropy is equivalent to the principle of a minimum of the K-L divergence. Here, the Gibbs inequality is written as ' -F(i,N)* log* F(i,N) <  -F(i,N)*log*W(i,N). The forms of entropy and rate functions for the ensemble are as follows, 'S(1b) =X*S(b)' and 'I(1b) =X*I^(b)'. Here both 'I(b)' and 'I(1b)' are non-negative (> 0).
 
%{For Quasi-Independent and Indistinguishable Systems}

For the quasi-independent and indistinguishable systems, we use the correct form of a joint spatial probability distribution and repeat the procedure from equations  2 to 4. The joint spatial distribution 'P(b)' and its natural logarithm, entropy, and rate functions are given below
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))= S(b)/k',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=- I^(b)'.

% Cramer-Chernoff Upper Bound for Total Internal Energy and Total Number of Particles
%Quasi-Independent and Distinguishable Systems

Now, let us consider the distribution of the macroscopic random variables of the state, the total internal energy 'E(t)' and the total number of particles 'N(t)'. The ensemble exchanges energy to a heat reservoir of temperature 'T' and particles to the particle reservoir of the chemical potential 'M'. 
To obtain the large deviation bound, the generalized form of the Bienayme-Chebyshev-Markov (BCM) probability inequality is used.  This generalized probability inequality expresses in terms of the moment generating function (MGF) or partition function and given thresholds of the random variables.
For the given random variables 'E(t)' and 'N(t)' of the ensemble, we define a new non-negative, real-valued exponential variable 'e^(-B(E(t)-M N(t))' with two real-valued parameters 'B' ('=1/kT') and the chemical potential 'M'. 
In the case of quasi-independent and distinguishable systems, Cramer and Chernoff large deviation upper bound 'P*(c)'  on the probability of 'e^(-B(E(t)-M N(t))' expresses in terms of the grand canonical partition function and the given thresholds on the energies and number of particles in the systems,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where 'B > 0', 'Z(B, M)' and 'Z(g)=(Z(B, M))^(X(t))' are the grand canonical partition functions of a single system and the ensemble respectively.
The symbol 'E' in the upper line of equation 6 denotes the mathematical expectation. 
The natural logarithm on both sides of 6, and then division on both sides by 'X(t)', supply
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.  
In equation 9, the limit X(t) to infinity exists. We know that the grand canonical entropy is proportional to the natural logarithm of the probability function 'P*(c)'. 
Equations 7 and 8 give the grand canonical entropies of the ensemble and single distinguishable system respectively, 'S*(c)=k*log*P*(c)=X(t)*[B*E- B*MN + log*Z(B,M)]' and 'S(E, N) =S*(c)/X(t) = k*[B*E+A*N + log*Z(B, A)]', where 'A = -B*M'. The Cramer-Chernoff  large deviation rate function for a single distinguishable system is 'I(E, N) =[-B*E-A*N- log*Z(B, A)] = [(B*G-E)- A*N] ', where the function 'G(B,A)=-(B^(-1))*log*Z(B,A)' is the Gibbs free energy. The rate function 'I(E, N)' shows duality with the Massieu potential function or Planck's characteristic function 'P(B,A)' '(= -B*G =log*Z(B,A)' through the Legendre-Fenchel transform 'log*Z(B, A) =[-B*E-A*N- I(E, N)]'. The rate function the grand canonical ensemble is written as 'I(N)= X(t)*I(E, N)'. We observe that the The Cramer-Chernoff large deviation rate function 'I(c)' or 'I1(E, N)' is identical to the Gibbs index of probability 'N'.  


%Quasi-Independent and Indistinguishable Systems
In the case of quasi-independent and indistinguishable systems, we put the correct form of the grand canonical partition function of the ensemble 'e^(-B*E(t)-M*N(t))/X(t)!' into equation 6 and then follow the steps of calculations of equations 7, and 8. In this case, the Crammer-Chernoff upper bound 'P*(c)' and its natural logarithm, and grand canonical entropy and rate functions are written as
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.
From equation 10, we get the total grand canonical entropy of the ensemble 'S*(c)= k*log*P*(c) = X(t)*S(1c),', where 'S(E, N)=k*[B*E+A*N +log*(eZ/X(t))]' is the entropy of a single indistinguishable system. The Cramer-Chernoff large deviation function for a single indistinguishable system is 'I(E, N)=-k*[B*E+A*N +log*(eZ/X(t))]'.  

%Statistical Equilibrium Condition for the Open Systems
The method of Lagrange's undetermined multipliers subject to restrictive conditions gives the most probable set of the systems 'X(i, N)' for each 'i' at the statistical equilibrium. The entropy or the logarithmic probability function attains the maximum value at the statistical equilibrium. In equations 4 and 8, the entropies $ 'S(b)' and S*(c) are functions of 'X(i,N)'. At the statistical equilibrium, the differentials of logarithmic functions 'dP(b)' and 'dP*(c)', or equivalently the differentials of entropies 'dS(b)' and 'dS*(c)', subject to the variations of the three constraints X=0, Y=0, and Z=0, vanish. 
Following the method of Lagrange's undetermined multipliers, we equate the total variations 'd' of equations 3 and 7 with respect to 'X(i, N)' to zero 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.
where, 'e^(B*G)=1/Z' ,. For the equal values of 'W(N)', we get the probability of finding a distinguishable system in a state with energy 'E(i)' and number of particles 'N(i)', 'X(i,N)/X(t) = e^(- B*E(i)-M*N(i))/Z(B,A)'. By utilizing the total variations of equations 5 and 10, we can obtain a similar expression as that of equation 12, for the probability of finding an indistinguishable system. However, the differences in the Boltzmann-Sanov and grand canonical entropies for indistinguishable and distinguishable cases are functions of 'X(t)'. 

The substitution of 'X(i, N)' from equation 13 into three constraints equation 2 furnishes the expressions for the grand partition function, mean energy, and mean number of particles per system respectively 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.
Using the expressions of 'E*' and 'N*' from 13 in equation 7, the mean grand-canonical entropy per system 'S(c) = S*(c)/X(t)', is,
'S(c) =k[B*E+A*N+ log*Z^(g)]', 
'X=kk[B*E+A*N+ log*Z^(g)]'. 
The recent study of the large deviations shows the connections of entropies or rate function, in terms of equalities and inequalities, with other thermodynamical variables in the reversible and irreversible processes.  
For the reversible processes, the differential of the total Boltzmann-Sanov entropy 'S(b)' shows equality with the differentials of Gibbs free energy and the mean work-done and inequality for the irreversible spatial arrangements of the systems. On the other hand, in the reversible process of the energy and particle with the reservoirs, the differential of total grand canonical entropy establishes equality with differentials of total mean internal energy, total work, and total mean number of particles, 'dS*(c)=B*dQ(c)= B*[dE*(c)+dW(c)-M*dN(c)]'. Both processes of spatial arrangements of the systems and the exchange process of the energy and particle with the reservoirs produce entropy. The entropy productions are zero (always positive) in the reversible (irreversible) processes of spatial arrangements of the open systems and energy and particle exchange with the respective reservoirs. The change in the total entropy of the grand ensemble occurs either due to the production of entropy in the spatial arrangements of open systems inside the ensemble or entropy exchange to or from the heat and particle reservoir. These assertions establish equalities (inequalities) of the total entropy production in the reversible (irreversible) processes of the spatial arrangements and energy-particle exchange 'dS(j)= dS(b)+dS(c)>0'. The upper line of equation 16 shows a strong similarity with the generalized form of the second law of thermodynamics that developed for the black-hole entropy. The middle and lower lines are the equalities (inequalities) of the entropy productions in the reversible (irreversible) diffusion processes that occur interior and exterior of the grand canonical ensemble.

%\sectionLarge Deviations for Spatial and Energy Distributions of Various Systems
Here, we study the large deviations for the distributions of macroscopic variables of various systems such as Planck's and Fermi's ideal linear oscillators, classical and quantum ideal gases, and the magnetic system of particles with spin. Previous studies on these systems utilized the Boltzmann's distribution for the spatial arrangements of members of a system and determined the most probable values using Lagrange's method of undetermined multipliers subject to the restrictive conditions on the total numbers of members and total energy of the system. Moreover, these studies ignored the BCM type probability inequality either for the total internal energy or for both the total number of particles and the total internal energy of the whole ensemble. 

To obtain large deviation results for each of the systems mentioned here, we repeat the following steps: (1) Follow the restrictive conditions and construct the joint spatial distribution for the members of a system and then, by taking the natural logarithm of spatial distribution and using Stirling's approximation for the factorials, obtain Boltzmann-Sanov entropy and rate functions for the macro-state a system and its member. (2) Calculate first the Cramer-Chernoff large deviation probability upper bound either on the total energy or both total numbers of members and the total energy of a system and then use of the natural logarithm of probability function and Stirling's approximation for the factorials provide the entropy and rate functions for the macro-state a system and its member. (3) Establish the statistical equilibrium condition from the differentials of either Boltzmann-Sanov and canonical or grand canonical entropies or the large deviation rate functions by using Lagrange's method of undetermined multipliers and by following the total variation of restrictive conditions on the total energy and total numbers of members of a system. 

% up to here.
%Planck Case: System of the Ideal Linear Oscillators
Planck considered a distribution of the ideal linear oscillators over the infinitesimal region elements of the state-space of the whole system. The notations are similar to those of Planck's book and his research articles. Let '(N=N1+N2+...+N(n)+...)' and '(E=E1+E2+...+E(n)+...)' be the total number of oscillators and the total energy of a system respectively. The subscript 'n' denotes the labeled region elements '(1,2,...,n,....)' of the state-space of a system. The variables 'N(n)' and 'E(n)' are the number of oscillators and their energies in the 'n-th' region respectively. The energy 'E(n)' of the 'N(n)' oscillators with the equal frequency 'f' in the 'n-th' region is 'E(n)=N(n)*(n-1/2)*h*f =  N*w(n)*(n-1/2)h*f', where 'h' is Planck's constant and 'w = Nn/N' is a distribution density. Here, the term '(n-1/2)*h*f' is the arithmetic mean of energies '(n-1)*h*f' and 'n*h*f' of the oscillators in the 'n-th' region. One can also take arithmetic mean over 'n' and 'n+1' region elements; then energy becomes 'E(n)=N(n)*(n+1/2)*h*f'. Moreover, the total energy 'E' of the whole system is the sum of energies of oscillators in all region elements  'E = N*h*f *(n-1/2)*w(n)', where 'w(n) = N(n)/N' is a probability. We can rewrite the total energy as 'E = N*U*', where 'U* = (n-1/2)*w(n)*h*f' is the mean energy per oscillator. 

Following step (1) and the constraints on the total number and total energy of the oscillators, we write large deviations results for the joint spatial distribution of the 'N' quasi-independent linear oscillators over all the region elements
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where 'N(n) > 0', 'w(n)=N(n)/N', '0< w(n)<1', and 'w(n)=1'. From equation 16, the total Boltzmann-Sanov entropy of the system is  'S(bp) = k*log*P(bp) ~ k*[N(n)*log*N - N(n)*log*N(n)]'. Besides, equation 18 gives the entropy of a single ideal oscillator is the mean logarithm of 'w(n)', 'S(bp)= S(bp)/N = -k*[w(n)*log*w(n)]=-k*(<log*w(n)>)'. The Boltzmann-Sanov rate functions for the system and single oscillator are negative of their respective entropies.

Step (2) gives the Cramer-Chernoff large deviation upper bound for the exponential variable of the total energy 'E' of the system. 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
Here 'B>0' and the symbol 'E' in equation 18 denotes the mathematical expectation, and 'Z1(B)=e^(-B*E1)' and 'Z(B)=e^(-B*E)=(e^(-B^E1))^(N)' are the partition functions, respectively, of the single oscillator and the whole system. The equations 19 and 20 supply the expressions, respectively, for the total canonical entropy of the system and the canonical entropy per oscillator 'S*(cp)=k*log*P*(cp) = k *[B*N*U+ N*log*Z1] ' and 'S(cp) = S*(cp)/N=k*[B*N*U+ N*log*Z1]'. For the system and an oscillator, the Cramer-Chernoff large deviation rate functions are 'I=-S/k' and 'I1=S1/k'.

At the statistical equilibrium, the 'd' variations of the entropies with respect to 'N(n)' vanish i.e. 'dS(bp) =0' and 'dS*(cp) =0'. We follow step (3) and get the statistical equilibrium condition for the most probable set of Planck's linear oscillators,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
where the partition function of an oscillator, 'Z1(B)=e^(-B*(n-1/2)*h*N)', is obtained by putting 21 in the condition 'N=N(n)'. Therefore, from equation 21, 'w(n)=e^(-B*(n-1/2)*h*N)' is the probability of finding exactly 'N(n)' oscillators in the 'n-th' region element. To obtain equation 21, we can also consider 'd' variations of equations 17 and 20 with respect to 'w(n)' and follow Lagrange's method of undetermined multipliers.
Using equation 21, the mean energy, 'U*' and mean entropy per oscillator 'S(cp)'  are written, respectively, as
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 

Planck defined a large positive number, the integer 'R' that measures the energy of the system of oscillators, 'R= (E/h*f) -(N/2)=(n-1)*N(n)'. Therefore, by step (1), for a given energy of the system, the joint spatial distribution of 'N' oscillators or the total number of distinct ways of assigning 'R' quanta to 'N' oscillators is
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
Follow step (2) and the Cramer-Chernoff upper bound of the total energy of the system of oscillators is  
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where we have put 'N*U=Rh*ft. The term 'Z1(B)' is the partition function of a single oscillator. Planck replaced the total energy 'E= N*U' of a system of 'N' oscillators with the discrete energy packets of large positive number 'R' (quanta) with finite equal quantity 'h*N', i.e. X=Y/N. Thus, 'E/N=U/N', where 'hu/2' is the zero-point energy.
By considering step (3), for the statistical equilibrium condition, the variations 'dR' of both sides of equations 24 and 26 vanish. 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
The mean energy per oscillator 'E/N' 
E(n)/N=(X*R*N+X)*h*N.

%Bose Case: System of Light Quanta
Let us consider Bose's famous work on the statistics of light quanta. Bose obtained the probability distribution of the light quanta that lie into the various cells of the phase-space of the whole system. Moreover, he reproduced Planck's results of the total entropy of the thermodynamic state and total energy density of the system of the light quanta. We apply steps (1) to (3) sequentially and obtain the large deviations for the distributions of the number of the light quanta and their energies.  The chemical potential 'm' is zero for a system of the light quanta. Here, we follow similar notations found in Bose's work.

Let 'As=Ps,r' be the total number of labeled cells '(Ps0,Ps1,....,P(s,r),...)' in the 's-th' infinitesimal frequency interval 'df'. The index 'r' indicates the number of light quanta in the cells of 'df' . The total number of light quanta and their total energy in the cells of 'df' are 'N(s)=P(s,r)' and 'E(s)=Ps*r*h*fs'  respectively.  These quantities per cell are written as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'
where 'w(r) =Ps,r/As' is a probability, and 'b*' and 'U*(sb)' are, respectively, the mean number of light quanta and their mean energy per cell of 'df'.
Step (1) provides the results for the joint distribution of the cells containing the various number of light quanta in 'df'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
The mean energy per oscillator 'E/N' 
E(n)/N=(X*R*N+X)*h*N.
The distribution over all infinitesimal frequency intervals is the product of distributions, 'P(bb)=W(bb)'. From, 31 and 32, we write the total Boltzmann-Sanov entropy 'S(bb)', and entropy per cell 'S(bb)/As' respectively.
'S(bb) = k *log*W(bb) ~ k *log*(As/P(s,r))', 
S(bb) = k *log*W(bb) ~ k *log*(As/P(s,r))'. 
Moreover, the total entropy of the system over all infinitesimal frequency intervals is 'S(bb) =S(bb)'. The Boltzmann-Sanov rate function are 'I(bb) =-S(bb)' and 'I1(bb) =-S1(bb)'
Considering step (2), for 'B>0, we have expressions for the Cramer-Chernoff large deviation upper bound on the probability of the total energy 'E(s)' of the light quanta, the natural logarithm of probability function, the canonical entropy and Cramer-Chernoff rate function in the interval 'df'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where '(Z(1,b))^(As)' is the partition function over all 'As' cells. The chemical potential 'M' is zero for the system of the light quanta. The distribution over all infinitesimal frequency intervals is 'P*(c)b=W(bb)'  
Equations 34 and 36 provide the expressions for the total canonical entropy 'S(sb)' and entropy per cell 'S(sb)/As' respectively.
'S(cb)= k *log*W(cb) = [k*B*r*fs + k*r*log*Z(1,b)]', 
'S(cb)= k *log*W(cb) = [k*B*r*fs + k*r*log*Z(1,b)]'. 
Following step (3), the equilibrium condition  is obtained by equating the deviations 'd' on both sides of equations 31 and 35 either with respect to 'ps,r' or with respect to 'w(s,r)' to zero. Here we equate 'dP(s,r)' to zero,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
where the partition function 'Z(1,b)(B)= e^(-B*r*h*fs)= (1-e^(-B*h*fs))^(-1)' is obtained from the condition 'r=0*P(s,r)= As'. The lower line of equation 38 gives the probability of exactly 'r' number of light quanta that lie in the cells of the interval 'df'. 
Using equation 38, the mean number of light quanta per cell in 'df'  is 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
This is identical with Planck's result (See equation 28).
Moreover, 'N*b=bs= e^(B*h*fs -1)' is the total mean occupancy number of the system of light quanta. 
Using equation 38, the total energy 'E(s)' and energy of the light quanta  per cell in 'df' are obtained, respectively, as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The energy of the whole system of light quanta over all the frequency intervals is 'E(b)=E(s)=B(s)', . 
The mean Gibbs canonical entropy in 'df' at the equilibrium ,is, 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
where in the second line of equation 41, we have put 'U*(sb)' from equation 40 and logarithm of 'Z(1,b)'. Moreover, the mean Gibbs canonical entropy per cell ,in 'df' from the last line of equation 41 is 
X*S(cb)*As = X*B*h*fs*e^(-B*h*fs-1*log*(1- e^(-B*h*fs)).
Equation 43 is identical to equation 23.
The entropy of the whole system of light quanta over all the frequency intervals is 'S(cb) =M*S(cb)'. 

%Fermi Case: System of Simple Oscillators
Schroedinger studied a simple system of the Fermi oscillators with zero chemical potential. Here the notations are identical to those of Bose's case. The Pauli exclusion principle restricts the number of oscillators (particles) per cell i.e. either  'r=0' or 'r=1' in each cell. The restrictive conditions are defined on the total number of cells 'As', total number of Fermi oscillators 'N(f)' and their energies 'E(f)' in the 's-th' interval, 'As = p(s)', 'N(s)=r*p(s)' and 'E(s)=r*e*p(s)', where 'e' is the energy of a single Fermi oscillator.

Step (1) gives us the joint spatial distribution 'W(bf)' of cells that filled with the oscillators, the total Boltzmann-Sanov entropy 'S(bf)' of the system, and entropy per cell 'S(bf)/As'. 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.'
The last line of equation 44 can be rewritten as 'k*log*W/A=S/A=k<log(w)> '.
We have the total spatial distribution for all the intervals 'P(bf)= W(bf)' and 'S(bf)=S(bf)'.
We consider step (2) and obtain the Cramer-Chernoff's large deviation bound, logarithmic probability function, canonical entropy for the total energy distribution of system of Fermi's oscillators 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
where 'B>0' and 'Z(1,f)=e^(-r*B*E)= (1+e^(-B*E))' is the partition function of a single Fermi oscillator respectively. For the whole system and all the intervals, we get 'P*(cf)=W(cf)' and 'S(cf)= S(cf)'. 
The use of step (3) provides the equilibrium condition for a system of the Fermi oscillators i.e. the most probable values of the oscillators. Equate the 'd' variations of the second line of equation 43 and the third line of equation 44 to zero.  
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
The lower line of equation 45 defines the probability of finding the Fermi oscillator in the cells of the 's' interval. Using this definition of the probability, equation 47, the mean occupation number of the oscillators per cell 'Sf' is given as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The total occupancy number is 'N*(f)=e^(B*E+1)'. 
Using equation 47, the total energy 'ESf' of oscillators and mean energy per cell and mean energy per cell 'U(sf)f' in the 's-th' interval are written as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'. 
Putting equation 47 in the mean entropy of oscillators and the mean entropy of oscillators per cell in the 's-th' interval, we get 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The total entropy of the system of the Fermi oscillators is 'Sf =N*S(cf)'.  

%Classical and Quantum Ideal Gases
In the previous sections, we have considered the systems of Planck and Fermi ideal linear oscillators, and light quanta with zero chemical potential. Here, we focus on the large deviations study for the distributions of the non-relativistic classical and quantum ideal gases with nonzero chemical potentials. The particles of the ideal gases obey three different types of statistics: (i) Maxwell-Boltzmann (MB) (ii) Bose-Einstein (BE), and (iii) Fermi-Dirac (FD). 
Due to weak interactions between the particles, they are assumed quasi-independent, and thus, the probabilities of macroscopic variables of the particles do not affect each other. Thus the problem of studying the statistics of macroscopic variables of the whole ideal gas reduces to that of studying the statistics of a single particle. Particles of the MB ideal gas are distinguishable and have no restrictions on occupancy in a single state. Bose-Einstein (BE) statistics allows any number of identical and indistinguishable particles (bosons) with integer spin in a single state. In the Fermi-Dirac ideal gas, a single state can not accommodate simultaneously more than one identical and indistinguishable particle (fermion) with half-integral spin because of the restriction of the Pauli exclusion principle. 
Quantum mechanically, the solution for the statistics of an ideal gas is to find the number of symmetric (antisymmetric) eigenfunctions for a boson (fermion) state. Let 'G(j)', 'N(j)', and 'E(j)' be the number of states, number of particles, and their energies in the 'j'-th group. The aggregate of the number of particles '(N(j), j=1,2,...)' into the states of the independent labeled groups 'j=1,2,...' defines the macroscopic state of the whole ideal gas. The total number of particles and total energy of the ideal gas are written as 'N(j)= Nt' and 'N(j)*E(j) = Et'. 

Our first aim is to find the distribution of the 'N(j)' particles that lie into the 'G(j)' states in the 'j'-th group and then in succession construct a distribution for all the independent groups of states. This is equivalent to finding the statistical weight i.e. the number of distinct ways 'G(j)' of distributing 'N(j)' particles over a state in the 'j-th' group. The total statistical weight for all the independent groups of the identical particles is the product of 'G(j)', i.e 'Pb(ig)^(G(j))'.  

Following step (1), the total statistical weights or joint spatial distributions of the particles of the three different types of ideal gases, satisfying the constraints on the total numbers of particles and total energy of the ideal gas, are written as  
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The total entropy of an ideal gas is proportional to the natural logarithm of the total statistical weight i.e. 'S(g) ~ k*log*P(ig)= k**log*G(j)'. 
'S(g) ~ k*log*P(ig)= k**log*G(j)',
'S(g) ~ k*log*P(ig)= k**log*G(j)',  
'S(g) ~ k*log*P(ig)= k**log*G(j)'.  
The use of step (2) gives us the Cramer-Chernoff large deviation upper bound on the probability of the variable 'e^(-B*E(t)-M*N(t))', the grand canonical entropy, and the Cramer-Chernoff rate function. 
'P*(c)< e^(-B*E(t)-M*N(t))',
'P*(c)< e^(-B*E(t)-M*N(t))', 
'P*(c)< e^(-B*E(t)-M*N(t))'.
where 'Zg(B,M)' is a grand partition function of whole ideal gas 
and 'A= -B*M'.  We put 'N(t) =N(j)' and 'N(t)U = N(j) E(j) ', and the logarithms of the grand partition functions for the MB, BE, and FD ideal gases in equation 53.
'log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',
'log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'.
We know that the grand canonical entropy for a macroscopic state of an ideal gas is proportional to the natural logarithm of a probability distribution, 'S*(ig) ~k*log*P*(ig); thus, 'S*(ig)= k*log*P*(ig) = S(ig)'. 
Consider step (3), the variations 'dN(j)' on both sides of the set of equations 51 and 54 provide the statistical equilibrium conditions for the set of most probable or mean values of the particles in the three different types of ideal gases.
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',  
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'. 
we get the mean occupation number of the particles in each of the state of 'j-th' group.
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',  
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'. 
The total mean occupancy number of the particles in an ideal gas is 'N=N*(j)'. 

%Magnetic System: Particles with Spins
The absolute temperature 'T' or the parameter 'B=1/kT' is nonnegative, i.e. 'T > 0' or 'B > 0', for for the closed or open normal thermodynamical system.  The internal energy of a normal system varies from zero (0) or a certain least attainable value, say E(+0) to the infinity ('I').
Here we follow steps (1) to (3) and study the large deviations for the distributions of numbers of particles and the total energy of a magnetic system. The internal energy of a magnetic system has both the lower 'Em,+0' and upper 'E-0' bounds, respectively,  for the temperatures 'T tends to +0' and 'T tends to -0'. 

Consider a magnetic system of 'N' weakly interacting quasi-independent particles with a spin '1/2'. This magnetic system is placed in the external magnetic field 'H'; thus, each of the particles has two orientations with a magnetic moment either '+M' parallel to or '-M' antiparallel to the field 'H'. Moreover, the corresponding non-degenerate energies are '+e=+u*H' and  '-e=-u*H'. 
The total number of particles 'N' and the total internal energy 'E' of a system are written as 'N=N++N-' and 'E=(N+-N-)M*H = M*E' respectively, where 'N+' and 'N-' are, respectively, the '+' spin and '-' spin particles, and 'M=N+-N-' is the magnetization. The numbers N+' and 'N-' are expressed in terms of 'M' and 'E' as follows 'N+ = (N+M)/2 = (N*E+E)/2*E ' and 'N- = (N-M)/2 = (N*E-E)/2*E'.    

%For the cases of normal closed or open systems, the temperature 'T' or 'B=1/kT' is nonnegative i.e. 'T > 0' or 'B > 0'. The internal energy of the normal systems or an ensemble varies from '0' (or a certain least attainable value, say 'E+') to 'I'. For the positive attainable temperature 'T > ' or 'B > 0', the internal energy 'E' lie in the interval '(E0, E+] ', where 'E+'  is the maximum value for maximum temperature 'T to infinity ' or 'B tends to +0'. As the temperature 'T tends +0 ' or to least value, then the internal of a system shifts to 'E0', and entropy attains its minimum value. This is the case of the third law of thermodynamics.  The magnetic system of particles with spins is in completely different thermodynamical states for the positive 'T > 0' ('B > 0') and negative 'T < 0' ('B < 0') temperatures. Moreover, at these temperatures, the entropy of the system attains the minimum value but for two entirely different thermodynamics states. Here we study the large deviations for the distributions of the magnetic system corresponding to both positive and negative temperatures. Let 'N+' and 'N-' be, respectively, '+' spin and '-' spin particles. The total number of particles 'N' and the total energy 'E' of the system are written as 'N=N++N-' and 'E=(N+-N-)M H = ME', where 'M=N+-N-' and '*E=M H' respectively. Therefore, we have This system is always termed a 'two-level system'.

By step (1), the number of ways of the spatial arrangements of the N+' and 'N-'  particles in the energy states '+e' and '-e' the thermodynamic weight 'Pb' of a macroscopic state of a magnetic system takes the final form 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',  
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'. 

In the last line of Eq.58, 'w- = X*N/N' and 'w+=X*N/N' are the probabilities. The Boltzmann-Sanov type entropy ' S(mb)' is Boltzmann constant times the natural logarithm of '*log*P(mb)' i.e. 'S(mb)= k *log*P(mb)'. By putting the values of 'N-' and 'N+' in equation 58, we have the expressions for the total Boltzmann-Sanov type entropy of a system and entropy per particle
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N', 
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N'.

From equation 59, the temperature 'T' of the system is defined as '1/T = dS/dE=(k/*E)*log[(N*E-E)/(N*E+E)]' or '1/T=(k/*E)*log(N+/N-)'. This temperature is either positive or negative according to whether 'N*e < E' or 'N*e > E' 
The parameter 'T* =-1/T' covers the entire range of temperature from '+infinity' to '-infinity' including zero. Table 1 shows the values of 'T', internal energy 'E', and entropy 'S' of a system at various temperatures. The magnetic system is in a completely different thermodynamical states for the positive 'T > 0' ('B > 0') and negative 'T < 0' ('B < 0') temperatures. Moreover, at these temperatures, the entropy of a  system attains the minimum value, but for the entirely different thermodynamical states. In the case of positive temperature, the population in the higher energy state is small 'N(-) <N(+)', whereas for the negative temperature the population is large 'N(-) >N(+)'.
In the experiment on the LiF crystal, by reversing the magnetic field, the thermodynamic equilibrium with the population 'N(-) >N(+)' in the maximum energy state was achieved successfully for the negative temperature. 

We now calculate the Crammer Chernoff upper bound on the probability inequality of the total internal energy 'E' of a system that exceeds to certain threshold 'Nu', where u is the energy per particle. Since the magnetic system exhibits different behavior for both positive and temperature, therefore the maximums of the Crammer Chernoff rate functions are achieved for the intervals of positive and negative temperature with the corresponding ranges of the total internal energies. Therefore we need two probability inequalities for the two intervals of positive and negative temperature. In this case, the population, number of particles, in the maximum energy state is larger than the minimum energy state.

(i) For a  strictly positive temperature 'T >0' ('T* < 0') and corresponding range of the total internal energy of the system, 'Em,+0< E < N*u', we define the probability inequality of the total internal energy and the given threshold 'P*(c)+(E < N*u)=P*(c)+(-E > -N*u)=P*(c)+(-B*E > -B N*u)', where 'B > 0'. (ii)In the case of the negative temperature 'T < 0' ('T*> 0')  and respective range of the total internal energy of a system 'Nu < E < E-0', we get another probability inequality of the total internal energy and the given threshold, 'P*(c)-(E > N*u)=P*(c)-(-B*E > -B*N*u)', where 'B < 0'. Then in the both regimes of positive and negative temperatures of the magnetic system, following step (1), the Cramer-Chernoff large deviation upper bounds and their natural logarithms, canonical entropies and rate functions are written as
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N', 
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N'.
Here the partition function of the whole system is the product of partition functions of the quasi-independent weakly interacting particles. In addition, the Helmholtz free energy of the system is 'A= -N*k*T*log*Z1 = -N*k*T*log(2*cosh(B*E))'. 

Consider step (3) and obtain the statistical equilibrium condition by equating the variations 'd' on sides of the equations 59 and 61 with respect to 'N-' and 'N+'  to zero.
S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N', 
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N'.
The upper and lower lines of equation 62 define the probabilities of finding a single particle of the magnetic system, respectively, in the states 'E+ =M*H' and 'E-=-M*H'. 
The mean energies of a particle and the system are given as 'U* = -d*log(Z1)/dB = -*E*tanh(B*E)' and 'E= M*E= (N+-E-)*E = - N*E*tanh(B*E)=N*U' respectively. 
Moreover, the mean entropies of the system and per particle are, respectively, obtained as 'S(cm) = B*N*U*+N*log*Z(1) = N*k*[-B*E*tanh(B*E)+log(2*cosh(B*E)]' and 'S(mc)= S(cm)/N*k = -B*E*tanh(B*E+log(2*cosh(B*E))'.



%The thermodynamic states of the system at temperatures 'T tends to +_infinity ' are identical. For these temperatures, the internal energy reaches to the mean values 'E +_ infinity' and the entropy attains the maximums 'Sm,+_infinity= N*k*log2'.The parameter 'T* =-1/T' captures all ranges from positive to negative temperatures. 

%For the cases of closed or open normal thermodynamical systems, the temperature $T$ or $\beta=1/kT$ is nonnegative i.e. $T \geq 0$ or $\beta \geq 0$ \cite{LandauV5,Haar95,Schroedinger13,Pathria11,Greiner95}. The internal energy of the normal systems or an ensemble varies from $0$ (or a certain least attainable value, say $E_{+0}$) to $\infty$ \cite{LandauV5,Haar95,Schroedinger13,Pathria11,Greiner95}.  Here we study the large deviations for the distributions of the magnetic system corresponding to both positive and negative temperatures.  The magnetic system of particles with spins is in completely different thermodynamical states for the positive $T \geq 0$ ($\beta \geq 0$) and negative $T \leq 0$ ($\beta \leq 0$) temperatures \cite{Ramsey56,Purcell51}. The internal energy of a magnetic system has lower $\mathsf{E}_{min,+0}$ and upper $\mathsf{E}_{max,-0}$ bounds, respectively, as $T \to +0$ and $T \to -0$ \cite{Ramsey56,Purcell51}. Moreover, at these temperatures, the entropy of the system attains the minimum value but for two entirely different thermodynamics states \cite{Ramsey56,Purcell51}.


\sectionDiscussions and Summary

\bibliographyGrandRef

\enddocument
%
% ****** End of file apstemplate.tex ******



==> LDT-BP/Grammarly1.tex <==
Large Deviation Statistics for the Distributions of Open Systems, Ideal Linear Oscillators, Light Quanta, Ideal Gases, and Magnetic System
D. P. Shinde
168-A, Panchsheel Colony, Pachgaon, Kolhapur, State-Maharashtra, India - 416013.
dpshinde.physics@gmail.com

We apply the large deviations theorems of Boltzmann-Sanov and Cramer-Chernoff, respectively, to the distributions of the spatial arrangements and the total number of particles and total internal energy of the open systems. The entropies obtained from both theorems are negative of their respective large deviation rate functions. We have found that the inequality (equality) of the total entropy change of the grand ensemble for the irreversible (reversible) processes of the spatial arrangements of systems and energy-particle exchange with the reservoirs are analogous to that of the generalized second law of thermodynamics. We extend the applications of large deviation statistics for the macroscopic variables of systems of the ideal Planck's and Fermi's linear oscillators, light quanta, ideal gases, and particles with spin. By Lagrange's method of undetermined multipliers, the sets of the most probable or mean values of the members of a system are obtained for a statistical equilibrium.

The asymptotic methods are essential for the constructions of limit theorems, laws of large numbers, and various convergence criteria for the sums of random variables. Besides, in general, these topics are very useful to understand the relevance of the mathematical theory of probability in all branches of science. In statistical physics, the distributions of internal energies and numbers of systems, considered as macroscopic random variables, of an ensemble, under generalized conditions, follow the central limit theorem (CLT) or Laplace-Gauss law of probability. The normal deviations of internal energies and numbers of systems from their respective mean values considered by CLT are used for understanding the states of equilibrium of the systems and ensemble. The modern large deviation theory (LDT) in its simple mathematical form or abstract probability measure-theoretic form determines the asymptotic probabilities and their decay rates for the random variables in rare events. 
However, physicists did not utilize the combination of Boltzmann-Sanov and Cramer-Chernoff large deviations theorems for the distributions of spatial arrangements of systems and their internal energies. A comparative study of the large deviations for the macroscopic variables of the distinguishable and indistinguishable systems has not been done. On the other hand, mathematical studies on the large deviations consider neither specific physical models of an isolated ensemble and ensemble-heat reservoir, respectively, for the distributions of spatial arrangements and the total internal energy of closed systems nor the reversible and irreversible diffusion processes of matter and energy. Besides, clear and coherent physical interpretations or inferences on the connections of large deviation entropies or rate functions with the laws of thermodynamics, relative fluctuations in the entropies, and entropy productions in the thermodynamical processes have not been shown.

Following Lagrange's method of undetermined multipliers, the D-variations of entropies with respect to the numbers of systems (particles) of an ensemble (an ideal gas) for the state of statistical equilibrium should vanish subject to the restrictive conditions, 'S(1)-S(2)=0'. 
This statistical equilibrium condition provides the mean or most probable set of values for the numbers of systems (particles) of an ensemble (an ideal gas). The entropies 'S1' and 'S2' are proportional to their respective logarithms of the probability distributions. The entropy 'S(1)=k*logP1+constant' is obtained from the joint or multinomial spatial probability distribution 'P1' of the systems subject to some constraints on the macroscopic variables of the ensemble. But, following the restrictive conditions on the total numbers of systems 'N' and total internal energy 'E' of an ensemble, the entropy 'S(2)=A+B'is directly written in terms of Lagrange's undetermined multipliers 'A' and 'B'. The parameters 'A' and 'B'. are related, respectively, to the inverses of a partition function 'Z' and the absolute temperature 'T'. However, for the entropy 'S(2)', the form of probability distribution was unknown. 

The recent study on the large deviations for the probability distributions distributions 'P1' and 'P2' of the random variables of closed systems has shown that a correct combination of the Boltzmann-Sanov and Cramer-Chernoff theorems provide the statistical equilibrium condition via Lagrange's method of undetermined multipliers. It shows clear and coherent interpretations of the large deviations results for the distributions of spatial arrangements and the internal energies of the closed systems. In particular, the spatial distribution of the systems 'P1' is obtained at a constant total energy of the closed and isolated ensemble whereas the distribution 'P2' is defined as probability inequality for the total internal energy of the ensemble at the constant total number of systems. Moreover, it has been shown that the large deviations results on the entropies or rate functions are connected in terms of equalities and inequalities, analogous to the laws of thermodynamics,  with the other thermodynamical variables in both reversible and irreversible diffusion processes of matter and energy. It is clearly stated that the large deviation rate functions are identical either to Boltzmann's 'H' or to Gibbs 'E' function. Furthermore, in the case of the coupled model of the ensemble and the heat reservoir, the physical significance of the large deviations results for the study of the relative fluctuations in the entropies is also illustrated.

%The modern large deviation theory (LDT) calculates the asymptotic probabilities of independent and dependent random variables beyond their normal deviations, exponential decay rates of probabilities, and determines the various mathematical properties of the rate functions. However, previous studies on the large deviations for the physical systems ignore the correct combination of Boltzmann-Sanov and Cramer-Chernoff theorems for determining the statistical equilibrium condition for the distributions of numbers of systems and their internal energies.  In particular, in the statistical equilibrium condition, Lagrange's undetermined parameters A and B are directly written from the restrictive conditions on the total number of systems and total internal energy of the ensemble. These parameters appear naturally by following the Cramer-Chernoff bound on the probability inequality for the total internal energy of the ensemble. Besides, the clear, continuous, and coherent physical interpretations on the connections of large deviation entropies or rate functions with the laws of thermodynamics have not been shown. Particularly, the logical connections of large deviations entropies or rate functions in terms of equalities and inequalities with other thermodynamical variables or functions are completely missing in previous studies. Furthermore, the use of large deviation theory for the relative fluctuations of entropies in case of coupling of ensemble and heat reservoir, and entropy productions in the irreversible diffusion processes of matter and energy are not studied. Mathematical studies on the large deviations consider neither specific physical models of an isolated ensemble and ensemble-heat reservoir for the distributions of spatial arrangements and the total internal energy of closed systems nor the reversible and irreversible diffusion processes of matter and energy. Most importantly, the physical interpretations or meanings of the known results on the large deviations and their various terms are not clearly stated in previous mathematical studies. 

%However, for the determination of the statistical equilibrium condition, previous studies on the large deviations for the physical systems ignore the correct combination of Boltzmann-Sanov and Cramer-Chernoff theorems, respectively, for the distributions of spatial arrangements of systems and their internal energies. Besides, the clear, continuous, and coherent physical interpretations on the connections of large deviation entropies or rate functions with the laws of thermodynamics have not been shown. In particular, the logical connections of large deviations entropies or rate functions in terms of equalities and inequalities with other thermodynamical variables or functions in the reversible and irreversible processes are completely missing in the previous studies. Furthermore, the use of large deviation theory for the relative fluctuations of entropies for the coupled of ensemble and heat reservoir, and for the entropy productions in the irreversible diffusion processes of matter and energy are not studied. Mathematical studies on the large deviations consider neither specific physical models of an isolated ensemble and ensemble-heat reservoir for the distributions of spatial arrangements and the total internal energy of closed systems nor the reversible and irreversible diffusion processes of matter and energy. Moreover, the physical significance or meaning of the known results on the large deviations is not stated for the information about states of physical systems. 

An ensemble is an imaginary collection of a large number of identical copies of a system that has a resemblance with the actual physical system. Three major types of ensembles, micro-canonical, canonical, and grand canonical are useful to study the thermodynamical properties of the classical and quantum physical systems. For these ensembles, various macroscopic variables and the state functions are defined for an individual system and the whole ensemble in their respective state spaces. For the given macro-states, the systems of the three ensembles have similar sets of values of their respective macroscopic variables. The sum of macroscopic variables of the systems defines a macroscopic variable for a certain macro-state of the whole ensemble. In equilibrium statistical mechanics, the ensemble averaging technique i.e. the averaging of a macroscopic variable over a large number of systems of an ensemble is equivalent to the time averaging technique for the same macroscopic variable. The systems of the micro-canonical ensemble are closed and isolated from the surroundings whereas the closed systems of canonical ensemble exchange only energy to the heat reservoir. 
The grand canonical ensemble consists of open systems which exchange both energy and particles with the heat and particle reservoirs respectively. To obtain the probability distribution of an unspecified open system, Gibbs defined a probability-coefficient 'Pg' and the index of probability 'N= *log*P(g)' as a function of macroscopic variables, the total internal energy, and the total number of particles of the grand canonical ensemble. Following Gibbs, for the grand canonical ensemble, we have 'P(g)=e^(O-E*T)', and 'N=log*P(g)= (O-E)/T', where 'T=1/kT' ('k' is Boltzmann constant and 'T' is absolute temperature), and 'M's are chemical potential of the components of the grand canonical ensemble. 

The large deviations of the general open systems and other various classical and quantum systems have not been studied. We plan our large deviation study on these systems as follows.
In the general case, we study the large deviations for the random variables, the numbers, and internal energies, of the large numbers of open classical systems of the grand canonical ensemble. In particular, we apply, respectively, the Boltzmann-Sanov theorem, for the joint spatial distributions of open systems of an isolated ensemble and the Cramer-Chernoff theorem for the distribution of the total internal energy and the total number of particles of the ensemble that couples to the heat and particle reservoirs. Moreover, in both cases, we obtain the entropy and rate functions for the macro-state of the ensemble. Furthermore, we suggest inequality (equality), analogous to the generalized second law of thermodynamics, of total entropy change of the grand ensemble in irreversible (reversible) processes of spatial arrangements of open systems and energy-particle exchange to the reservoirs. The thorough large deviation analysis gives the entropies and rate functions for the distributions of the spatial arrangements and energies of Planck's and Fermi's ideal linear oscillators, light quanta, particles of the ideal gases, and the particles with spins. For all these case studies, we obtain the statistical equilibrium conditions using the method of Lagrange undetermined multipliers. 

%In equilibrium statistical mechanics, the ensemble averaging technique i.e. the averaging of a macroscopic variable over a large number of systems of the ensemble is equivalent to the time averaging technique for the same macroscopic variable. Moreover, these ensemble theories are applicable to study the statistics of the macroscopic variables of systems of ideal linear oscillators, light quanta, classical and quantum ideal gases, and particles with spins. In the statistical equilibrium, the distributions of macroscopic variables such as internal energies and numbers of the systems of particles in the systems, under the generalized conditions, asymptotically follow the Laplace-Gauss or normal probability law. The deviations from the respective mean values of macroscopic variables, following the normal law, are called the normal deviations. To obtain the joint spatial distribution of the various open systems and distribution of the total internal energy and the total number of particles of the ensemble, respectively, the ensemble is isolated from its surroundings and is attached to the heat and particle reservoirs.
 
%This article, following the Boltzmann-Sanov theorem, provides large deviations for the joint spatial distribution of open systems, and the entropy and rate functions for the macro-state of the grand canonical ensemble. Besides, we use Cramer-Chernoff's theorem for calculations of the large deviation upper bound on the probability, the entropy, and the rate functions for the total internal energy and the total number of particles of the ensemble. The thorough large deviation analysis gives the entropies and rate functions for the distributions of the spatial arrangements and energies of Planck's and Fermi's ideal linear oscillators, light quanta, particles of the ideal gases, and the particles with spins. For all these case studies, we obtain the statistical equilibrium conditions using the method of Lagrange undetermined multipliers. 

{General Case: Large Deviations for Open Systems} 
%In the general case, we study the large deviations of the random variables, the numbers and internal energies, of the open classical systems of the grand canonical ensemble. In particular, we apply, respectively, the Boltzmann-Sanov theorem, for the joint spatial distributions of open systems of an isolated ensemble and Cramer-Chernoff theorem for the distribution of the total internal energy and the total number of particles of the ensemble which couple with the heat and particle reservoirs. The grand canonical ensemble consists of very large number X of macroscopic, quasi-independent, distinguishable or indistinguishable open systems.
{Joint or Multinomial Spatial Distribution: For Quasi-Independent Distinguishable Systems}

First, we construct a joint or multinomial spatial distribution of a very large number 'X(t)' of macroscopic, quasi-independent, and distinguishable systems at a given set of values of (T, V, m), where V is the volume and then repeating the same procedure, write down large deviations results for the quasi-independent and indistinguishable systems. 

At any given instant of time, let 'X(i, N)' be the number of systems having the number of particles 'N'  and energy 'E(i)' in the states of an 'i-th' partition. The subscripts 'i' and 'N' denote, respectively, an 'i-th' partition of the phase-space of the whole ensemble and the number of particles in a system. The energy 'E(i)' of the system in the given macro-state varies with the number of particles. The macroscopic variables 'X(i, N)', 'N', and 'E(i)', regarded as random variables, of the states, fluctuate about their respective mean values. The probability of finding an unspecified open system of a grand ensemble in a particular macro-state depends on a certain amount of energy and the number of particles of that macro-state. This is also defined as a ratio of the number of systems 'X(i, N)' that lies in the states an 'i'-th partition to the total number of systems 'X(t)'. Let 'W(N)' denotes a probability of finding a single system in any one of the states of an 'i'-th partition with the energy 'E(i)' and the number of particles 'N'. Then, the occupation probability of 'X(i, N)' systems in the states of an 'i'-th partition is
'W,(N)X(i,N)'. The macroscopic configuration '(X(i, N);i=1,...,r)' of spatial arrangements of all systems over the states of all the partitions, following some restrictive conditions, can be realized in a number of ways. This is also known as the joint or multinomial spatial distribution of all the systems subject to restrictive conditions. The three restrictive conditions fix the total number of systems 'X(t)', total internal energy 'E(t)', and the total number of particles 'N(t)' of the ensemble. 
These restrictive conditions are defined in the following way
(i)N*X(i,N)= X(t), (ii)N*E(i)X(i,N)=X(t)E*=E(t), i(ii),N*N(i)*X(i,N)=X(t)N* =N(t),
where 'X(i,N)> 0', 'E(i)> 0', 'N(i)> 0'. The ratios 'E*=E(t)/X(t)' and 'N*=N(t)/X(t)', respectively, the mean energy and mean number of the particles per system remain constants in the infinite limits of 'E(t)', 'N(t)', and 'X(t)'. The sum in equation2 is the double sum and it runs over 'i' and 'N'. The use of combinatorics, satisfying the equation 2, provides the final form of the joint spatial distribution 'P(b)' of the quasi-independent and distinguishable systems 
'P(b)(X(i,N);i=1,...,)= X!*[W(N)^X(i,N)/X(i,N)!]', 
where '0 < W(N) < 1' and 'W(N)=1'. 
Now first, we take the natural logarithm on both sides of equation 2 and then use Stirling's approximation for the factorials of large numbers 'X! ~ X*log*X-X' and 'X(i,N)! ~ X(i,N) *log*X(i,N) -X(i,N)'. Thus, we get the equations
'log*P(b)(.)=log*X ! + [X(i,N)*log*W(N)-log*X(i,N)!]',
'log*P(b)(.)=log*X ! + [X(i,N)*log*W(N)-log*X(i,N)!]'.
The total Boltzmann-Sanov entropy 'S(b)' of the ensemble is proportional to the logarithm of the probability function 'log*P(b)'. Therefore, from the lower line of equation 3, we have the expression for the entropy 'S(b) = k*log*P(b)', where k is the Boltzmann constant. Dividing on both sides of the lower line of equation 3 by 'X', we have,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'X*log*P(b)(.) ~ F(i,N)*log*(W(N)/F(i,N))',
where 'F(i,N) =X(i,N)/X' is the ratio of the number of systems that fall in the 'i-th' partition to the total number of systems, and 'F(i,N)=1'. The thermodynamic limit 'X to infinity for 'X/*log*P(b)(.)' exists and from the lower line of equation 4, the function 'S(b)=F(i,N)*log*(W(N)/F(i,N))' is the Boltzmann-Sanov entropy of a single system. In addition, it is a sum of cross entropy and the entropy of mixing. In this case of joint spatial distribution, the Boltzmann-Sanov rate function for a single system is negative of its entropy (negentropy) function, 'I(b)=-S(b)=F(i,N)*log(F(i,N)/W(N)) = [F(i,N)*W(N)*log*(F(i,N)/W(N))]'. 

Entropy, probability function, and information are linked to each other. The rate function 'I(F, W)' is also known as Kullback-Leibler (K-L) divergence or discrimination information between 'F' and 'W'. If 'W' refers to the relative volume of a partition and approximates F then I(F, W) (negentropy) is the information loss about the system's state. A principle of the maximum of entropy is equivalent to the principle of a minimum of the K-L divergence. Here, the Gibbs inequality is written as ' -F(i,N)* log* F(i,N) <  -F(i,N)*log*W(i,N). The forms of entropy and rate functions for the ensemble are as follows, 'S(1b) =X*S(b)' and 'I(1b) =X*I^(b)'. Here both 'I(b)' and 'I(1b)' are non-negative (> 0).
 
%{For Quasi-Independent and Indistinguishable Systems}

For the quasi-independent and indistinguishable systems, we use the correct form of a joint spatial probability distribution and repeat the procedure from equations  2 to 4. The joint spatial distribution 'P(b)' and its natural logarithm, entropy, and rate functions are given below
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))= S(b)/k',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=- I^(b)'.

% Cramer-Chernoff Upper Bound for Total Internal Energy and Total Number of Particles
%Quasi-Independent and Distinguishable Systems

Now, let us consider the distribution of the macroscopic random variables of the state, the total internal energy 'E(t)' and the total number of particles 'N(t)'. The ensemble exchanges energy to a heat reservoir of temperature 'T' and particles to the particle reservoir of the chemical potential 'M'. 
To obtain the large deviation bound, the generalized form of the Bienayme-Chebyshev-Markov (BCM) probability inequality is used.  This generalized probability inequality expresses in terms of the moment generating function (MGF) or partition function and given thresholds of the random variables.
For the given random variables 'E(t)' and 'N(t)' of the ensemble, we define a new non-negative, real-valued exponential variable 'e^(-B(E(t)-M N(t))' with two real-valued parameters 'B' ('=1/kT') and the chemical potential 'M'. 
In the case of quasi-independent and distinguishable systems, Cramer and Chernoff large deviation upper bound 'P*(c)'  on the probability of 'e^(-B(E(t)-M N(t))' expresses in terms of the grand canonical partition function and the given thresholds on the energies and number of particles in the systems,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where 'B > 0', 'Z(B, M)' and 'Z(g)=(Z(B, M))^(X(t))' are the grand canonical partition functions of a single system and the ensemble respectively.
The symbol 'E' in the upper line of equation 6 denotes the mathematical expectation. 
The natural logarithm on both sides of 6, and then division on both sides by 'X(t)', supply
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.  
In equation 9, the limit X(t) to infinity exists. We know that the grand canonical entropy is proportional to the natural logarithm of the probability function 'P*(c)'. 
Equations 7 and 8 give the grand canonical entropies of the ensemble and single distinguishable system respectively, 'S*(c)=k*log*P*(c)=X(t)*[B*E- B*MN + log*Z(B,M)]' and 'S(E, N) =S*(c)/X(t) = k*[B*E+A*N + log*Z(B, A)]', where 'A = -B*M'. The Cramer-Chernoff  large deviation rate function for a single distinguishable system is 'I(E, N) =[-B*E-A*N- log*Z(B, A)] = [(B*G-E)- A*N] ', where the function 'G(B,A)=-(B^(-1))*log*Z(B,A)' is the Gibbs free energy. The rate function 'I(E, N)' shows duality with the Massieu potential function or Planck's characteristic function 'P(B,A)' '(= -B*G =log*Z(B,A)' through the Legendre-Fenchel transform 'log*Z(B, A) =[-B*E-A*N- I(E, N)]'. The rate function the grand canonical ensemble is written as 'I(N)= X(t)*I(E, N)'. We observe that the The Cramer-Chernoff large deviation rate function 'I(c)' or 'I1(E, N)' is identical to the Gibbs index of probability 'N'.  


%Quasi-Independent and Indistinguishable Systems
In the case of quasi-independent and indistinguishable systems, we put the correct form of the grand canonical partition function of the ensemble 'e^(-B*E(t)-M*N(t))/X(t)!' into equation 6 and then follow the steps of calculations of equations 7, and 8. In this case, the Crammer-Chernoff upper bound 'P*(c)' and its natural logarithm, and grand canonical entropy and rate functions are written as
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.
From equation 10, we get the total grand canonical entropy of the ensemble 'S*(c)= k*log*P*(c) = X(t)*S(1c),', where 'S(E, N)=k*[B*E+A*N +log*(eZ/X(t))]' is the entropy of a single indistinguishable system. The Cramer-Chernoff large deviation function for a single indistinguishable system is 'I(E, N)=-k*[B*E+A*N +log*(eZ/X(t))]'.  

%Statistical Equilibrium Condition for the Open Systems
The method of Lagrange's undetermined multipliers subject to restrictive conditions gives the most probable set of the systems 'X(i, N)' for each 'i' at the statistical equilibrium. The entropy or the logarithmic probability function attains the maximum value at the statistical equilibrium. In equations 4 and 8, the entropies $ 'S(b)' and S*(c) are functions of 'X(i,N)'. At the statistical equilibrium, the differentials of logarithmic functions 'dP(b)' and 'dP*(c)', or equivalently the differentials of entropies 'dS(b)' and 'dS*(c)', subject to the variations of the three constraints X=0, Y=0, and Z=0, vanish. 
Following the method of Lagrange's undetermined multipliers, we equate the total variations 'd' of equations 3 and 7 with respect to 'X(i, N)' to zero 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.
where, 'e^(B*G)=1/Z' ,. For the equal values of 'W(N)', we get the probability of finding a distinguishable system in a state with energy 'E(i)' and number of particles 'N(i)', 'X(i,N)/X(t) = e^(- B*E(i)-M*N(i))/Z(B,A)'. By utilizing the total variations of equations 5 and 10, we can obtain a similar expression as that of equation 12, for the probability of finding an indistinguishable system. However, the differences in the Boltzmann-Sanov and grand canonical entropies for indistinguishable and distinguishable cases are functions of 'X(t)'. 

The substitution of 'X(i, N)' from equation 13 into three constraints equation 2 furnishes the expressions for the grand partition function, mean energy, and mean number of particles per system respectively 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.
Using the expressions of 'E*' and 'N*' from 13 in equation 7, the mean grand-canonical entropy per system 'S(c) = S*(c)/X(t)', is,
'S(c) =k[B*E+A*N+ log*Z^(g)]', 
'X=kk[B*E+A*N+ log*Z^(g)]'. 
The recent study of the large deviations shows the connections of entropies or rate function, in terms of equalities and inequalities, with other thermodynamical variables in the reversible and irreversible processes.  
For the reversible processes, the differential of the total Boltzmann-Sanov entropy 'S(b)' shows equality with the differentials of Gibbs free energy and the mean work-done and inequality for the irreversible spatial arrangements of the systems. On the other hand, in the reversible process of the energy and particle with the reservoirs, the differential of total grand canonical entropy establishes equality with differentials of total mean internal energy, total work, and total mean number of particles, 'dS*(c)=B*dQ(c)= B*[dE*(c)+dW(c)-M*dN(c)]'. Both processes of spatial arrangements of the systems and the exchange process of the energy and particle with the reservoirs produce entropy. The entropy productions are zero (always positive) in the reversible (irreversible) processes of spatial arrangements of the open systems and energy and particle exchange with the respective reservoirs. The change in the total entropy of the grand ensemble occurs either due to the production of entropy in the spatial arrangements of open systems inside the ensemble or entropy exchange to or from the heat and particle reservoir. These assertions establish equalities (inequalities) of the total entropy production in the reversible (irreversible) processes of the spatial arrangements and energy-particle exchange 'dS(j)= dS(b)+dS(c)>0'. The upper line of equation 16 shows a strong similarity with the generalized form of the second law of thermodynamics that developed for the black-hole entropy. The middle and lower lines are the equalities (inequalities) of the entropy productions in the reversible (irreversible) diffusion processes that occur interior and exterior of the grand canonical ensemble.

%\sectionLarge Deviations for Spatial and Energy Distributions of Various Systems
Here, we study the large deviations for the distributions of macroscopic variables of various systems such as Planck's and Fermi's ideal linear oscillators, classical and quantum ideal gases, and the magnetic system of particles with spin. Previous studies on these systems utilized the Boltzmann's distribution for the spatial arrangements of members of a system and determined the most probable values using Lagrange's method of undetermined multipliers subject to the restrictive conditions on the total numbers of members and total energy of the system. Moreover, these studies ignored the BCM type probability inequality either for the total internal energy or for both the total number of particles and the total internal energy of the whole ensemble. 

To obtain large deviation results for each of the systems mentioned here, we repeat the following steps: (1) Follow the restrictive conditions and construct the joint spatial distribution for the members of a system and then, by taking the natural logarithm of spatial distribution and using Stirling's approximation for the factorials, obtain Boltzmann-Sanov entropy and rate functions for the macro-state a system and its member. (2) Calculate first the Cramer-Chernoff large deviation probability upper bound either on the total energy or both total numbers of members and the total energy of a system and then use of the natural logarithm of probability function and Stirling's approximation for the factorials provide the entropy and rate functions for the macro-state a system and its member. (3) Establish the statistical equilibrium condition from the differentials of either Boltzmann-Sanov and canonical or grand canonical entropies or the large deviation rate functions by using Lagrange's method of undetermined multipliers and by following the total variation of restrictive conditions on the total energy and total numbers of members of a system. 

% up to here.
%Planck Case: System of the Ideal Linear Oscillators
Planck considered a distribution of the ideal linear oscillators over the infinitesimal region elements of the state-space of the whole system. The notations are similar to those of Planck's book and his research articles. Let '(N=N1+N2+...+N(n)+...)' and '(E=E1+E2+...+E(n)+...)' be the total number of oscillators and the total energy of a system respectively. The subscript 'n' denotes the labeled region elements '(1,2,...,n,....)' of the state-space of a system. The variables 'N(n)' and 'E(n)' are the number of oscillators and their energies in the 'n-th' region respectively. The energy 'E(n)' of the 'N(n)' oscillators with the equal frequency 'f' in the 'n-th' region is 'E(n)=N(n)*(n-1/2)*h*f =  N*w(n)*(n-1/2)h*f', where 'h' is Planck's constant and 'w = Nn/N' is a distribution density. Here, the term '(n-1/2)*h*f' is the arithmetic mean of energies '(n-1)*h*f' and 'n*h*f' of the oscillators in the 'n-th' region. One can also take arithmetic mean over 'n' and 'n+1' region elements; then energy becomes 'E(n)=N(n)*(n+1/2)*h*f'. Moreover, the total energy 'E' of the whole system is the sum of energies of oscillators in all region elements  'E = N*h*f *(n-1/2)*w(n)', where 'w(n) = N(n)/N' is a probability. We can rewrite the total energy as 'E = N*U*', where 'U* = (n-1/2)*w(n)*h*f' is the mean energy per oscillator. 

Following step (1) and the constraints on the total number and total energy of the oscillators, we write large deviations results for the joint spatial distribution of the 'N' quasi-independent linear oscillators over all the region elements
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where 'N(n) > 0', 'w(n)=N(n)/N', '0< w(n)<1', and 'w(n)=1'. From equation 16, the total Boltzmann-Sanov entropy of the system is  'S(bp) = k*log*P(bp) ~ k*[N(n)*log*N - N(n)*log*N(n)]'. Besides, equation 18 gives the entropy of a single ideal oscillator is the mean logarithm of 'w(n)', 'S(bp)= S(bp)/N = -k*[w(n)*log*w(n)]=-k*(<log*w(n)>)'. The Boltzmann-Sanov rate functions for the system and single oscillator are negative of their respective entropies.

Step (2) gives the Cramer-Chernoff large deviation upper bound for the exponential variable of the total energy 'E' of the system. 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
Here 'B>0' and the symbol 'E' in equation 18 denotes the mathematical expectation, and 'Z1(B)=e^(-B*E1)' and 'Z(B)=e^(-B*E)=(e^(-B^E1))^(N)' are the partition functions, respectively, of the single oscillator and the whole system. The equations 19 and 20 supply the expressions, respectively, for the total canonical entropy of the system and the canonical entropy per oscillator 'S*(cp)=k*log*P*(cp) = k *[B*N*U+ N*log*Z1] ' and 'S(cp) = S*(cp)/N=k*[B*N*U+ N*log*Z1]'. For the system and an oscillator, the Cramer-Chernoff large deviation rate functions are 'I=-S/k' and 'I1=S1/k'.

At the statistical equilibrium, the 'd' variations of the entropies with respect to 'N(n)' vanish i.e. 'dS(bp) =0' and 'dS*(cp) =0'. We follow step (3) and get the statistical equilibrium condition for the most probable set of Planck's linear oscillators,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
where the partition function of an oscillator, 'Z1(B)=e^(-B*(n-1/2)*h*N)', is obtained by putting 21 in the condition 'N=N(n)'. Therefore, from equation 21, 'w(n)=e^(-B*(n-1/2)*h*N)' is the probability of finding exactly 'N(n)' oscillators in the 'n-th' region element. To obtain equation 21, we can also consider 'd' variations of equations 17 and 20 with respect to 'w(n)' and follow Lagrange's method of undetermined multipliers.
Using equation 21, the mean energy, 'U*' and mean entropy per oscillator 'S(cp)'  are written, respectively, as
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 

Planck defined a large positive number, the integer 'R' that measures the energy of the system of oscillators, 'R= (E/h*f) -(N/2)=(n-1)*N(n)'. Therefore, by step (1), for a given energy of the system, the joint spatial distribution of 'N' oscillators or the total number of distinct ways of assigning 'R' quanta to 'N' oscillators is
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
Follow step (2) and the Cramer-Chernoff upper bound of the total energy of the system of oscillators is  
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where we have put 'N*U=Rh*ft. The term 'Z1(B)' is the partition function of a single oscillator. Planck replaced the total energy 'E= N*U' of a system of 'N' oscillators with the discrete energy packets of large positive number 'R' (quanta) with finite equal quantity 'h*N', i.e. X=Y/N. Thus, 'E/N=U/N', where 'hu/2' is the zero-point energy.
By considering step (3), for the statistical equilibrium condition, the variations 'dR' of both sides of equations 24 and 26 vanish. 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
The mean energy per oscillator 'E/N' 
E(n)/N=(X*R*N+X)*h*N.

%Bose Case: System of Light Quanta
Let us consider Bose's famous work on the statistics of light quanta. Bose obtained the probability distribution of the light quanta that lie into the various cells of the phase-space of the whole system. Moreover, he reproduced Planck's results of the total entropy of the thermodynamic state and total energy density of the system of the light quanta. We apply steps (1) to (3) sequentially and obtain the large deviations for the distributions of the number of the light quanta and their energies.  The chemical potential 'm' is zero for a system of the light quanta. Here, we follow similar notations found in Bose's work.

Let 'As=Ps,r' be the total number of labeled cells '(Ps0,Ps1,....,P(s,r),...)' in the 's-th' infinitesimal frequency interval 'df'. The index 'r' indicates the number of light quanta in the cells of 'df' . The total number of light quanta and their total energy in the cells of 'df' are 'N(s)=P(s,r)' and 'E(s)=Ps*r*h*fs'  respectively.  These quantities per cell are written as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'
where 'w(r) =Ps,r/As' is a probability, and 'b*' and 'U*(sb)' are, respectively, the mean number of light quanta and their mean energy per cell of 'df'.
Step (1) provides the results for the joint distribution of the cells containing the various number of light quanta in 'df'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
The mean energy per oscillator 'E/N' 
E(n)/N=(X*R*N+X)*h*N.
The distribution over all infinitesimal frequency intervals is the product of distributions, 'P(bb)=W(bb)'. From, 31 and 32, we write the total Boltzmann-Sanov entropy 'S(bb)', and entropy per cell 'S(bb)/As' respectively.
'S(bb) = k *log*W(bb) ~ k *log*(As/P(s,r))', 
S(bb) = k *log*W(bb) ~ k *log*(As/P(s,r))'. 
Moreover, the total entropy of the system over all infinitesimal frequency intervals is 'S(bb) =S(bb)'. The Boltzmann-Sanov rate function are 'I(bb) =-S(bb)' and 'I1(bb) =-S1(bb)'
Considering step (2), for 'B>0, we have expressions for the Cramer-Chernoff large deviation upper bound on the probability of the total energy 'E(s)' of the light quanta, the natural logarithm of probability function, the canonical entropy and Cramer-Chernoff rate function in the interval 'df'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where '(Z(1,b))^(As)' is the partition function over all 'As' cells. The chemical potential 'M' is zero for the system of the light quanta. The distribution over all infinitesimal frequency intervals is 'P*(c)b=W(bb)'  
Equations 34 and 36 provide the expressions for the total canonical entropy 'S(sb)' and entropy per cell 'S(sb)/As' respectively.
'S(cb)= k *log*W(cb) = [k*B*r*fs + k*r*log*Z(1,b)]', 
'S(cb)= k *log*W(cb) = [k*B*r*fs + k*r*log*Z(1,b)]'. 
Following step (3), the equilibrium condition  is obtained by equating the deviations 'd' on both sides of equations 31 and 35 either with respect to 'ps,r' or with respect to 'w(s,r)' to zero. Here we equate 'dP(s,r)' to zero,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
where the partition function 'Z(1,b)(B)= e^(-B*r*h*fs)= (1-e^(-B*h*fs))^(-1)' is obtained from the condition 'r=0*P(s,r)= As'. The lower line of equation 38 gives the probability of exactly 'r' number of light quanta that lie in the cells of the interval 'df'. 
Using equation 38, the mean number of light quanta per cell in 'df'  is 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
This is identical with Planck's result (See equation 28).
Moreover, 'N*b=bs= e^(B*h*fs -1)' is the total mean occupancy number of the system of light quanta. 
Using equation 38, the total energy 'E(s)' and energy of the light quanta  per cell in 'df' are obtained, respectively, as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The energy of the whole system of light quanta over all the frequency intervals is 'E(b)=E(s)=B(s)', . 
The mean Gibbs canonical entropy in 'df' at the equilibrium ,is, 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
where in the second line of equation 41, we have put 'U*(sb)' from equation 40 and logarithm of 'Z(1,b)'. Moreover, the mean Gibbs canonical entropy per cell ,in 'df' from the last line of equation 41 is 
X*S(cb)*As = X*B*h*fs*e^(-B*h*fs-1*log*(1- e^(-B*h*fs)).
Equation 43 is identical to equation 23.
The entropy of the whole system of light quanta over all the frequency intervals is 'S(cb) =M*S(cb)'. 

%Fermi Case: System of Simple Oscillators
Schroedinger studied a simple system of the Fermi oscillators with zero chemical potential. Here the notations are identical to those of Bose's case. The Pauli exclusion principle restricts the number of oscillators (particles) per cell i.e. either  'r=0' or 'r=1' in each cell. The restrictive conditions are defined on the total number of cells 'As', total number of Fermi oscillators 'N(f)' and their energies 'E(f)' in the 's-th' interval, 'As = p(s)', 'N(s)=r*p(s)' and 'E(s)=r*e*p(s)', where 'e' is the energy of a single Fermi oscillator.

Step (1) gives us the joint spatial distribution 'W(bf)' of cells that filled with the oscillators, the total Boltzmann-Sanov entropy 'S(bf)' of the system, and entropy per cell 'S(bf)/As'. 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.'
The last line of equation 44 can be rewritten as 'k*log*W/A=S/A=k<log(w)> '.
We have the total spatial distribution for all the intervals 'P(bf)= W(bf)' and 'S(bf)=S(bf)'.
We consider step (2) and obtain the Cramer-Chernoff's large deviation bound, logarithmic probability function, canonical entropy for the total energy distribution of system of Fermi's oscillators 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
where 'B>0' and 'Z(1,f)=e^(-r*B*E)= (1+e^(-B*E))' is the partition function of a single Fermi oscillator respectively. For the whole system and all the intervals, we get 'P*(cf)=W(cf)' and 'S(cf)= S(cf)'. 
The use of step (3) provides the equilibrium condition for a system of the Fermi oscillators i.e. the most probable values of the oscillators. Equate the 'd' variations of the second line of equation 43 and the third line of equation 44 to zero.  
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
The lower line of equation 45 defines the probability of finding the Fermi oscillator in the cells of the 's' interval. Using this definition of the probability, equation 47, the mean occupation number of the oscillators per cell 'Sf' is given as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The total occupancy number is 'N*(f)=e^(B*E+1)'. 
Using equation 47, the total energy 'ESf' of oscillators and mean energy per cell and mean energy per cell 'U(sf)f' in the 's-th' interval are written as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'. 
Putting equation 47 in the mean entropy of oscillators and the mean entropy of oscillators per cell in the 's-th' interval, we get 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The total entropy of the system of the Fermi oscillators is 'Sf =N*S(cf)'.  

%Classical and Quantum Ideal Gases
In the previous sections, we have considered the systems of Planck and Fermi ideal linear oscillators, and light quanta with zero chemical potential. Here, we focus on the large deviations study for the distributions of the non-relativistic classical and quantum ideal gases with nonzero chemical potentials. The particles of the ideal gases obey three different types of statistics: (i) Maxwell-Boltzmann (MB) (ii) Bose-Einstein (BE), and (iii) Fermi-Dirac (FD). 
Due to weak interactions between the particles, they are assumed quasi-independent, and thus, the probabilities of macroscopic variables of the particles do not affect each other. Thus the problem of studying the statistics of macroscopic variables of the whole ideal gas reduces to that of studying the statistics of a single particle. Particles of the MB ideal gas are distinguishable and have no restrictions on occupancy in a single state. Bose-Einstein (BE) statistics allows any number of identical and indistinguishable particles (bosons) with integer spin in a single state. In the Fermi-Dirac ideal gas, a single state can not accommodate simultaneously more than one identical and indistinguishable particle (fermion) with half-integral spin because of the restriction of the Pauli exclusion principle. 
Quantum mechanically, the solution for the statistics of an ideal gas is to find the number of symmetric (antisymmetric) eigenfunctions for a boson (fermion) state. Let 'G(j)', 'N(j)', and 'E(j)' be the number of states, number of particles, and their energies in the 'j'-th group. The aggregate of the number of particles '(N(j), j=1,2,...)' into the states of the independent labeled groups 'j=1,2,...' defines the macroscopic state of the whole ideal gas. The total number of particles and total energy of the ideal gas are written as 'N(j)= Nt' and 'N(j)*E(j) = Et'. 

Our first aim is to find the distribution of the 'N(j)' particles that lie into the 'G(j)' states in the 'j'-th group and then in succession construct a distribution for all the independent groups of states. This is equivalent to finding the statistical weight i.e. the number of distinct ways 'G(j)' of distributing 'N(j)' particles over a state in the 'j-th' group. The total statistical weight for all the independent groups of the identical particles is the product of 'G(j)', i.e 'Pb(ig)^(G(j))'.  

Following step (1), the total statistical weights or joint spatial distributions of the particles of the three different types of ideal gases, satisfying the constraints on the total numbers of particles and total energy of the ideal gas, are written as  
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The total entropy of an ideal gas is proportional to the natural logarithm of the total statistical weight i.e. 'S(g) ~ k*log*P(ig)= k**log*G(j)'. 
'S(g) ~ k*log*P(ig)= k**log*G(j)',
'S(g) ~ k*log*P(ig)= k**log*G(j)',  
'S(g) ~ k*log*P(ig)= k**log*G(j)'.  
The use of step (2) gives us the Cramer-Chernoff large deviation upper bound on the probability of the variable 'e^(-B*E(t)-M*N(t))', the grand canonical entropy, and the Cramer-Chernoff rate function. 
'P*(c)< e^(-B*E(t)-M*N(t))',
'P*(c)< e^(-B*E(t)-M*N(t))', 
'P*(c)< e^(-B*E(t)-M*N(t))'.
where 'Zg(B,M)' is a grand partition function of whole ideal gas 
and 'A= -B*M'.  We put 'N(t) =N(j)' and 'N(t)U = N(j) E(j) ', and the logarithms of the grand partition functions for the MB, BE, and FD ideal gases in equation 53.
'log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',
'log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'.
We know that the grand canonical entropy for a macroscopic state of an ideal gas is proportional to the natural logarithm of a probability distribution, 'S*(ig) ~k*log*P*(ig); thus, 'S*(ig)= k*log*P*(ig) = S(ig)'. 
Consider step (3), the variations 'dN(j)' on both sides of the set of equations 51 and 54 provide the statistical equilibrium conditions for the set of most probable or mean values of the particles in the three different types of ideal gases.
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',  
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'. 
we get the mean occupation number of the particles in each of the state of 'j-th' group.
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',  
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'. 
The total mean occupancy number of the particles in an ideal gas is 'N=N*(j)'. 

%Magnetic System: Particles with Spins
The absolute temperature 'T' or the parameter 'B=1/kT' is nonnegative, i.e. 'T > 0' or 'B > 0', for for the closed or open normal thermodynamical system.  The internal energy of a normal system varies from zero (0) or a certain least attainable value, say E(+0) to the infinity ('I').
Here we follow steps (1) to (3) and study the large deviations for the distributions of numbers of particles and the total energy of a magnetic system. The internal energy of a magnetic system has both the lower 'Em,+0' and upper 'E-0' bounds, respectively,  for the temperatures 'T tends to +0' and 'T tends to -0'. 

Consider a magnetic system of 'N' weakly interacting quasi-independent particles with a spin '1/2'. This magnetic system is placed in the external magnetic field 'H'; thus, each of the particles has two orientations with a magnetic moment either '+M' parallel to or '-M' antiparallel to the field 'H'. Moreover, the corresponding non-degenerate energies are '+e=+u*H' and  '-e=-u*H'. 
The total number of particles 'N' and the total internal energy 'E' of a system are written as 'N=N++N-' and 'E=(N+-N-)M*H = M*E' respectively, where 'N+' and 'N-' are, respectively, the '+' spin and '-' spin particles, and 'M=N+-N-' is the magnetization. The numbers N+' and 'N-' are expressed in terms of 'M' and 'E' as follows 'N+ = (N+M)/2 = (N*E+E)/2*E ' and 'N- = (N-M)/2 = (N*E-E)/2*E'.    

%For the cases of normal closed or open systems, the temperature 'T' or 'B=1/kT' is nonnegative i.e. 'T > 0' or 'B > 0'. The internal energy of the normal systems or an ensemble varies from '0' (or a certain least attainable value, say 'E+') to 'I'. For the positive attainable temperature 'T > ' or 'B > 0', the internal energy 'E' lie in the interval '(E0, E+] ', where 'E+'  is the maximum value for maximum temperature 'T to infinity ' or 'B tends to +0'. As the temperature 'T tends +0 ' or to least value, then the internal of a system shifts to 'E0', and entropy attains its minimum value. This is the case of the third law of thermodynamics.  The magnetic system of particles with spins is in completely different thermodynamical states for the positive 'T > 0' ('B > 0') and negative 'T < 0' ('B < 0') temperatures. Moreover, at these temperatures, the entropy of the system attains the minimum value but for two entirely different thermodynamics states. Here we study the large deviations for the distributions of the magnetic system corresponding to both positive and negative temperatures. Let 'N+' and 'N-' be, respectively, '+' spin and '-' spin particles. The total number of particles 'N' and the total energy 'E' of the system are written as 'N=N++N-' and 'E=(N+-N-)M H = ME', where 'M=N+-N-' and '*E=M H' respectively. Therefore, we have This system is always termed a 'two-level system'.

By step (1), the number of ways of the spatial arrangements of the N+' and 'N-'  particles in the energy states '+e' and '-e' the thermodynamic weight 'Pb' of a macroscopic state of a magnetic system takes the final form 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',  
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'. 

In the last line of Eq.58, 'w- = X*N/N' and 'w+=X*N/N' are the probabilities. The Boltzmann-Sanov type entropy ' S(mb)' is Boltzmann constant times the natural logarithm of '*log*P(mb)' i.e. 'S(mb)= k *log*P(mb)'. By putting the values of 'N-' and 'N+' in equation 58, we have the expressions for the total Boltzmann-Sanov type entropy of a system and entropy per particle
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N', 
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N'.

From equation 59, the temperature 'T' of the system is defined as '1/T = dS/dE=(k/*E)*log[(N*E-E)/(N*E+E)]' or '1/T=(k/*E)*log(N+/N-)'. This temperature is either positive or negative according to whether 'N*e < E' or 'N*e > E' 
The parameter 'T* =-1/T' covers the entire range of temperature from '+infinity' to '-infinity' including zero. Table 1 shows the values of 'T', internal energy 'E', and entropy 'S' of a system at various temperatures. The magnetic system is in a completely different thermodynamical states for the positive 'T > 0' ('B > 0') and negative 'T < 0' ('B < 0') temperatures. Moreover, at these temperatures, the entropy of a  system attains the minimum value, but for the entirely different thermodynamical states. In the case of positive temperature, the population in the higher energy state is small 'N(-) <N(+)', whereas for the negative temperature the population is large 'N(-) >N(+)'.
In the experiment on the LiF crystal, by reversing the magnetic field, the thermodynamic equilibrium with the population 'N(-) >N(+)' in the maximum energy state was achieved successfully for the negative temperature. 

We now calculate the Crammer Chernoff upper bound on the probability inequality of the total internal energy 'E' of a system that exceeds to certain threshold 'Nu', where u is the energy per particle. Since the magnetic system exhibits different behavior for both positive and temperature, therefore the maximums of the Crammer Chernoff rate functions are achieved for the intervals of positive and negative temperature with the corresponding ranges of the total internal energies. Therefore we need two probability inequalities for the two intervals of positive and negative temperature. In this case, the population, number of particles, in the maximum energy state is larger than the minimum energy state.

(i) For a  strictly positive temperature 'T >0' ('T* < 0') and corresponding range of the total internal energy of the system, 'Em,+0< E < N*u', we define the probability inequality of the total internal energy and the given threshold 'P*(c)+(E < N*u)=P*(c)+(-E > -N*u)=P*(c)+(-B*E > -B N*u)', where 'B > 0'. (ii)In the case of the negative temperature 'T < 0' ('T*> 0')  and respective range of the total internal energy of a system 'Nu < E < E-0', we get another probability inequality of the total internal energy and the given threshold, 'P*(c)-(E > N*u)=P*(c)-(-B*E > -B*N*u)', where 'B < 0'. Then in the both regimes of positive and negative temperatures of the magnetic system, following step (1), the Cramer-Chernoff large deviation upper bounds and their natural logarithms, canonical entropies and rate functions are written as
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N', 
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N'.
Here the partition function of the whole system is the product of partition functions of the quasi-independent weakly interacting particles. In addition, the Helmholtz free energy of the system is 'A= -N*k*T*log*Z1 = -N*k*T*log(2*cosh(B*E))'. 

Consider step (3) and obtain the statistical equilibrium condition by equating the variations 'd' on sides of the equations 59 and 61 with respect to 'N-' and 'N+'  to zero.
S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N', 
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N'.
The upper and lower lines of equation 62 define the probabilities of finding a single particle of the magnetic system, respectively, in the states 'E+ =M*H' and 'E-=-M*H'. 
The mean energies of a particle and the system are given as 'U* = -d*log(Z1)/dB = -*E*tanh(B*E)' and 'E= M*E= (N+-E-)*E = - N*E*tanh(B*E)=N*U' respectively. 
Moreover, the mean entropies of the system and per particle are, respectively, obtained as 'S(cm) = B*N*U*+N*log*Z(1) = N*k*[-B*E*tanh(B*E)+log(2*cosh(B*E)]' and 'S(mc)= S(cm)/N*k = -B*E*tanh(B*E+log(2*cosh(B*E))'.



%The thermodynamic states of the system at temperatures 'T tends to +_infinity ' are identical. For these temperatures, the internal energy reaches to the mean values 'E +_ infinity' and the entropy attains the maximums 'Sm,+_infinity= N*k*log2'.The parameter 'T* =-1/T' captures all ranges from positive to negative temperatures. 

%For the cases of closed or open normal thermodynamical systems, the temperature $T$ or $\beta=1/kT$ is nonnegative i.e. $T \geq 0$ or $\beta \geq 0$ \cite{LandauV5,Haar95,Schroedinger13,Pathria11,Greiner95}. The internal energy of the normal systems or an ensemble varies from $0$ (or a certain least attainable value, say $E_{+0}$) to $\infty$ \cite{LandauV5,Haar95,Schroedinger13,Pathria11,Greiner95}.  Here we study the large deviations for the distributions of the magnetic system corresponding to both positive and negative temperatures.  The magnetic system of particles with spins is in completely different thermodynamical states for the positive $T \geq 0$ ($\beta \geq 0$) and negative $T \leq 0$ ($\beta \leq 0$) temperatures \cite{Ramsey56,Purcell51}. The internal energy of a magnetic system has lower $\mathsf{E}_{min,+0}$ and upper $\mathsf{E}_{max,-0}$ bounds, respectively, as $T \to +0$ and $T \to -0$ \cite{Ramsey56,Purcell51}. Moreover, at these temperatures, the entropy of the system attains the minimum value but for two entirely different thermodynamics states \cite{Ramsey56,Purcell51}.


\sectionDiscussions and Summary

\bibliographyGrandRef

\enddocument
%
% ****** End of file apstemplate.tex ******



==> LDT-BP/Grammarly2.tex <==
Large Deviation Statistics for the Distributions of Open Systems, Ideal Linear Oscillators, Light Quanta, Ideal Gases, and Magnetic System
D. P. Shinde
168-A, Panchsheel Colony, Pachgaon, Kolhapur, State-Maharashtra, India - 416013.
dpshinde.physics@gmail.com

We apply the large deviations theorems of Boltzmann-Sanov and Cramer-Chernoff, respectively, to the distributions of the spatial arrangements and the total number of particles and total internal energy of the open systems. The entropies obtained from both theorems are negative of their respective large deviation rate functions. We have found that the inequality (equality) of the total entropy change of the grand ensemble for the irreversible (reversible) processes of the spatial arrangements of systems and energy-particle exchange with the reservoirs are analogous to that of the generalized second law of thermodynamics. We extend the applications of large deviation statistics for the macroscopic variables of systems of the ideal Planck's and Fermi's linear oscillators, light quanta, ideal gases, and particles with spin. By Lagrange's method of undetermined multipliers, the sets of the most probable or mean values of the members of a system are obtained for a statistical equilibrium.


The asymptotic methods are essential for the constructions of limit theorems, laws of large numbers, and various convergence criteria for the sums of random variables. Besides, in general, these topics are very useful to understand the relevance of the mathematical theory of probability in all branches of science. In statistical physics, the distributions of internal energies and numbers of systems, considered as macroscopic random variables, of an ensemble, under generalized conditions, follow the central limit theorem (CLT) or Laplace-Gauss law of probability. The normal deviations of internal energies and numbers of systems from their respective mean values considered by CLT are used for understanding the states of equilibrium of the systems and ensemble. The modern large deviation theory (LDT) in its simple mathematical form or abstract probability measure-theoretic form determines the asymptotic probabilities and their decay rates for the random variables in rare events. 


However, the previous mathematical and physical studies on large deviations for distributions of the classical systems did not address the following points. 
I)A comparative study of large deviations for distinguishable and indistinguishable systems
ii)A formula for a probability occurrence of relative fluctuations in the Boltzmann-Sanov and Gibbs entropies for the non-isolated model of ensemble and heat-reservoir
iii)A connection between large deviation entropies or rate functions and the loss of heat or work or the Clausius uncompensated transformations ?
iv)A connection between large deviation entropies or rate functions to equality or inequality of the generalized second law of thermodynamics for the total entropy production, rather then ordinary form of second law of thermodynamics. 
V)The generalized De Donder type inequality for the entropy productions in the processes that occur interior and exterior of the ensemble



However, physicists did not utilize the combination of Boltzmann-Sanov and Cramer-Chernoff large deviations theorems for the distributions of spatial arrangements of systems and their internal energies. A comparative study of the large deviations for the macroscopic variables of the distinguishable and indistinguishable systems has not been done. On the other hand, mathematical studies on the large deviations consider neither specific physical models of an isolated ensemble and ensemble-heat reservoir, respectively, for the distributions of spatial arrangements and the total internal energy of closed systems nor the reversible and irreversible diffusion processes of matter and energy. Besides, clear and coherent physical interpretations or inferences on the connections of large deviation entropies or rate functions with the laws of thermodynamics, relative fluctuations in the entropies, and entropy productions in the thermodynamical processes have not been shown.

Following Lagrange's method of undetermined multipliers, the D-variations of entropies with respect to the numbers of systems (particles) of an ensemble (an ideal gas) for the state of statistical equilibrium should vanish subject to the restrictive conditions, 'S(1)-S(2)=0'. 
This statistical equilibrium condition provides the mean or most probable set of values for the numbers of systems (particles) of an ensemble (an ideal gas). The entropies 'S1' and 'S2' are proportional to their respective logarithms of the probability distributions. The entropy 'S(1)=k*logP1+constant' is obtained from the joint or multinomial spatial probability distribution 'P1' of the systems subject to some constraints on the macroscopic variables of the ensemble. But, following the restrictive conditions on the total numbers of systems 'N' and total internal energy 'E' of an ensemble, the entropy 'S(2)=A+B'is directly written in terms of Lagrange's undetermined multipliers 'A' and 'B'. The parameters 'A' and 'B'. are related, respectively, to the inverses of a partition function 'Z' and the absolute temperature 'T'. However, for the entropy 'S(2)', the form of probability distribution was unknown. 

The recent study on the large deviations for the probability distributions distributions 'P1' and 'P2' of the random variables of closed systems has shown that a correct combination of the Boltzmann-Sanov and Cramer-Chernoff theorems provide the statistical equilibrium condition via Lagrange's method of undetermined multipliers. It shows clear and coherent interpretations of the large deviations results for the distributions of spatial arrangements and the internal energies of the closed systems. In particular, the spatial distribution of the systems 'P1' is obtained at a constant total energy of the closed and isolated ensemble whereas the distribution 'P2' is defined as probability inequality for the total internal energy of the ensemble at the constant total number of systems. Moreover, it has been shown that the large deviations results on the entropies or rate functions are connected in terms of equalities and inequalities, analogous to the laws of thermodynamics,  with the other thermodynamical variables in both reversible and irreversible diffusion processes of matter and energy. It is clearly stated that the large deviation rate functions are identical either to Boltzmann's 'H' or to Gibbs 'E' function. Furthermore, in the case of the coupled model of the ensemble and the heat reservoir, the physical significance of the large deviations results for the study of the relative fluctuations in the entropies is also illustrated.

%The modern large deviation theory (LDT) calculates the asymptotic probabilities of independent and dependent random variables beyond their normal deviations, exponential decay rates of probabilities, and determines the various mathematical properties of the rate functions. However, previous studies on the large deviations for the physical systems ignore the correct combination of Boltzmann-Sanov and Cramer-Chernoff theorems for determining the statistical equilibrium condition for the distributions of numbers of systems and their internal energies.  In particular, in the statistical equilibrium condition, Lagrange's undetermined parameters A and B are directly written from the restrictive conditions on the total number of systems and total internal energy of the ensemble. These parameters appear naturally by following the Cramer-Chernoff bound on the probability inequality for the total internal energy of the ensemble. Besides, the clear, continuous, and coherent physical interpretations on the connections of large deviation entropies or rate functions with the laws of thermodynamics have not been shown. Particularly, the logical connections of large deviations entropies or rate functions in terms of equalities and inequalities with other thermodynamical variables or functions are completely missing in previous studies. Furthermore, the use of large deviation theory for the relative fluctuations of entropies in case of coupling of ensemble and heat reservoir, and entropy productions in the irreversible diffusion processes of matter and energy are not studied. Mathematical studies on the large deviations consider neither specific physical models of an isolated ensemble and ensemble-heat reservoir for the distributions of spatial arrangements and the total internal energy of closed systems nor the reversible and irreversible diffusion processes of matter and energy. Most importantly, the physical interpretations or meanings of the known results on the large deviations and their various terms are not clearly stated in previous mathematical studies. 

%However, for the determination of the statistical equilibrium condition, previous studies on the large deviations for the physical systems ignore the correct combination of Boltzmann-Sanov and Cramer-Chernoff theorems, respectively, for the distributions of spatial arrangements of systems and their internal energies. Besides, the clear, continuous, and coherent physical interpretations on the connections of large deviation entropies or rate functions with the laws of thermodynamics have not been shown. In particular, the logical connections of large deviations entropies or rate functions in terms of equalities and inequalities with other thermodynamical variables or functions in the reversible and irreversible processes are completely missing in the previous studies. Furthermore, the use of large deviation theory for the relative fluctuations of entropies for the coupled of ensemble and heat reservoir, and for the entropy productions in the irreversible diffusion processes of matter and energy are not studied. Mathematical studies on the large deviations consider neither specific physical models of an isolated ensemble and ensemble-heat reservoir for the distributions of spatial arrangements and the total internal energy of closed systems nor the reversible and irreversible diffusion processes of matter and energy. Moreover, the physical significance or meaning of the known results on the large deviations is not stated for the information about states of physical systems. 

An ensemble is an imaginary collection of a large number of identical copies of a system that has a resemblance with the actual physical system. Three major types of ensembles, micro-canonical, canonical, and grand canonical are useful to study the thermodynamical properties of the classical and quantum physical systems. For these ensembles, various macroscopic variables and the state functions are defined for an individual system and the whole ensemble in their respective state spaces. For the given macro-states, the systems of the three ensembles have similar sets of values of their respective macroscopic variables. The sum of macroscopic variables of the systems defines a macroscopic variable for a certain macro-state of the whole ensemble. In equilibrium statistical mechanics, the ensemble averaging technique i.e. the averaging of a macroscopic variable over a large number of systems of an ensemble is equivalent to the time averaging technique for the same macroscopic variable. The systems of the micro-canonical ensemble are closed and isolated from the surroundings whereas the closed systems of canonical ensemble exchange only energy to the heat reservoir. 
The grand canonical ensemble consists of open systems which exchange both energy and particles with the heat and particle reservoirs respectively. To obtain the probability distribution of an unspecified open system, Gibbs defined a probability-coefficient 'Pg' and the index of probability 'N= *log*P(g)' as a function of macroscopic variables, the total internal energy, and the total number of particles of the grand canonical ensemble. Following Gibbs, for the grand canonical ensemble, we have 'P(g)=e^(O-E*T)', and 'N=log*P(g)= (O-E)/T', where 'T=1/kT' ('k' is Boltzmann constant and 'T' is absolute temperature), and 'M's are chemical potential of the components of the grand canonical ensemble. 

The large deviations of the general open systems and other various classical and quantum systems have not been studied. We plan our large deviation study on these systems as follows.
In the general case, we study the large deviations for the random variables, the numbers, and internal energies, of the large numbers of open classical systems of the grand canonical ensemble. In particular, we apply, respectively, the Boltzmann-Sanov theorem, for the joint spatial distributions of open systems of an isolated ensemble and the Cramer-Chernoff theorem for the distribution of the total internal energy and the total number of particles of the ensemble that couples to the heat and particle reservoirs. Moreover, in both cases, we obtain the entropy and rate functions for the macro-state of the ensemble. Furthermore, we suggest inequality (equality), analogous to the generalized second law of thermodynamics, of total entropy change of the grand ensemble in irreversible (reversible) processes of spatial arrangements of open systems and energy-particle exchange to the reservoirs. The thorough large deviation analysis gives the entropies and rate functions for the distributions of the spatial arrangements and energies of Planck's and Fermi's ideal linear oscillators, light quanta, particles of the ideal gases, and the particles with spins. For all these case studies, we obtain the statistical equilibrium conditions using the method of Lagrange undetermined multipliers. 

%In equilibrium statistical mechanics, the ensemble averaging technique i.e. the averaging of a macroscopic variable over a large number of systems of the ensemble is equivalent to the time averaging technique for the same macroscopic variable. Moreover, these ensemble theories are applicable to study the statistics of the macroscopic variables of systems of ideal linear oscillators, light quanta, classical and quantum ideal gases, and particles with spins. In the statistical equilibrium, the distributions of macroscopic variables such as internal energies and numbers of the systems of particles in the systems, under the generalized conditions, asymptotically follow the Laplace-Gauss or normal probability law. The deviations from the respective mean values of macroscopic variables, following the normal law, are called the normal deviations. To obtain the joint spatial distribution of the various open systems and distribution of the total internal energy and the total number of particles of the ensemble, respectively, the ensemble is isolated from its surroundings and is attached to the heat and particle reservoirs.
 
%This article, following the Boltzmann-Sanov theorem, provides large deviations for the joint spatial distribution of open systems, and the entropy and rate functions for the macro-state of the grand canonical ensemble. Besides, we use Cramer-Chernoff's theorem for calculations of the large deviation upper bound on the probability, the entropy, and the rate functions for the total internal energy and the total number of particles of the ensemble. The thorough large deviation analysis gives the entropies and rate functions for the distributions of the spatial arrangements and energies of Planck's and Fermi's ideal linear oscillators, light quanta, particles of the ideal gases, and the particles with spins. For all these case studies, we obtain the statistical equilibrium conditions using the method of Lagrange undetermined multipliers. 

{General Case: Large Deviations for Open Systems} 
%In the general case, we study the large deviations of the random variables, the numbers and internal energies, of the open classical systems of the grand canonical ensemble. In particular, we apply, respectively, the Boltzmann-Sanov theorem, for the joint spatial distributions of open systems of an isolated ensemble and Cramer-Chernoff theorem for the distribution of the total internal energy and the total number of particles of the ensemble which couple with the heat and particle reservoirs. The grand canonical ensemble consists of very large number X of macroscopic, quasi-independent, distinguishable or indistinguishable open systems.
{Joint or Multinomial Spatial Distribution: For Quasi-Independent Distinguishable Systems}

First, we construct a joint or multinomial spatial distribution of a very large number 'X(t)' of macroscopic, quasi-independent, and distinguishable systems at a given set of values of (T, V, m), where V is the volume and then repeating the same procedure, write down large deviations results for the quasi-independent and indistinguishable systems. 

At any given instant of time, let 'X(i, N)' be the number of systems having the number of particles 'N'  and energy 'E(i)' in the states of an 'i-th' partition. The subscripts 'i' and 'N' denote, respectively, an 'i-th' partition of the phase-space of the whole ensemble and the number of particles in a system. The energy 'E(i)' of the system in the given macro-state varies with the number of particles. The macroscopic variables 'X(i, N)', 'N', and 'E(i)', regarded as random variables, of the states, fluctuate about their respective mean values. The probability of finding an unspecified open system of a grand ensemble in a particular macro-state depends on a certain amount of energy and the number of particles of that macro-state. This is also defined as a ratio of the number of systems 'X(i, N)' that lies in the states an 'i'-th partition to the total number of systems 'X(t)'. Let 'W(N)' denotes a probability of finding a single system in any one of the states of an 'i'-th partition with the energy 'E(i)' and the number of particles 'N'. Then, the occupation probability of 'X(i, N)' systems in the states of an 'i'-th partition is
'W,(N)X(i,N)'. The macroscopic configuration '(X(i, N);i=1,...,r)' of spatial arrangements of all systems over the states of all the partitions, following some restrictive conditions, can be realized in a number of ways. This is also known as the joint or multinomial spatial distribution of all the systems subject to restrictive conditions. The three restrictive conditions fix the total number of systems 'X(t)', total internal energy 'E(t)', and the total number of particles 'N(t)' of the ensemble. 
These restrictive conditions are defined in the following way
(i)N*X(i,N)= X(t), (ii)N*E(i)X(i,N)=X(t)E*=E(t), i(ii),N*N(i)*X(i,N)=X(t)N* =N(t),
where 'X(i,N)> 0', 'E(i)> 0', 'N(i)> 0'. The ratios 'E*=E(t)/X(t)' and 'N*=N(t)/X(t)', respectively, the mean energy and mean number of the particles per system remain constants in the infinite limits of 'E(t)', 'N(t)', and 'X(t)'. The sum in equation2 is the double sum and it runs over 'i' and 'N'. The use of combinatorics, satisfying the equation 2, provides the final form of the joint spatial distribution 'P(b)' of the quasi-independent and distinguishable systems 
'P(b)(X(i,N);i=1,...,)= X!*[W(N)^X(i,N)/X(i,N)!]', 
where '0 < W(N) < 1' and 'W(N)=1'. 
Now first, we take the natural logarithm on both sides of equation 2 and then use Stirling's approximation for the factorials of large numbers 'X! ~ X*log*X-X' and 'X(i,N)! ~ X(i,N) *log*X(i,N) -X(i,N)'. Thus, we get the equations
'log*P(b)(.)=log*X ! + [X(i,N)*log*W(N)-log*X(i,N)!]',
'log*P(b)(.)=log*X ! + [X(i,N)*log*W(N)-log*X(i,N)!]'.
The total Boltzmann-Sanov entropy 'S(b)' of the ensemble is proportional to the logarithm of the probability function 'log*P(b)'. Therefore, from the lower line of equation 3, we have the expression for the entropy 'S(b) = k*log*P(b)', where k is the Boltzmann constant. Dividing on both sides of the lower line of equation 3 by 'X', we have,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'X*log*P(b)(.) ~ F(i,N)*log*(W(N)/F(i,N))',
where 'F(i,N) =X(i,N)/X' is the ratio of the number of systems that fall in the 'i-th' partition to the total number of systems, and 'F(i,N)=1'. The thermodynamic limit 'X to infinity for 'X/*log*P(b)(.)' exists and from the lower line of equation 4, the function 'S(b)=F(i,N)*log*(W(N)/F(i,N))' is the Boltzmann-Sanov entropy of a single system. In addition, it is a sum of cross entropy and the entropy of mixing. In this case of joint spatial distribution, the Boltzmann-Sanov rate function for a single system is negative of its entropy (negentropy) function, 'I(b)=-S(b)=F(i,N)*log(F(i,N)/W(N)) = [F(i,N)*W(N)*log*(F(i,N)/W(N))]'. 

Entropy, probability function, and information are linked to each other. The rate function 'I(F, W)' is also known as Kullback-Leibler (K-L) divergence or discrimination information between 'F' and 'W'. If 'W' refers to the relative volume of a partition and approximates F then I(F, W) (negentropy) is the information loss about the system's state. A principle of the maximum of entropy is equivalent to the principle of a minimum of the K-L divergence. Here, the Gibbs inequality is written as ' -F(i,N)* log* F(i,N) <  -F(i,N)*log*W(i,N). The forms of entropy and rate functions for the ensemble are as follows, 'S(1b) =X*S(b)' and 'I(1b) =X*I^(b)'. Here both 'I(b)' and 'I(1b)' are non-negative (> 0).
 
%{For Quasi-Independent and Indistinguishable Systems}

For the quasi-independent and indistinguishable systems, we use the correct form of a joint spatial probability distribution and repeat the procedure from equations  2 to 4. The joint spatial distribution 'P(b)' and its natural logarithm, entropy, and rate functions are given below
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))= S(b)/k',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=- I^(b)'.

% Cramer-Chernoff Upper Bound for Total Internal Energy and Total Number of Particles
%Quasi-Independent and Distinguishable Systems

Now, let us consider the distribution of the macroscopic random variables of the state, the total internal energy 'E(t)' and the total number of particles 'N(t)'. The ensemble exchanges energy to a heat reservoir of temperature 'T' and particles to the particle reservoir of the chemical potential 'M'. 
To obtain the large deviation bound, the generalized form of the Bienayme-Chebyshev-Markov (BCM) probability inequality is used.  This generalized probability inequality expresses in terms of the moment generating function (MGF) or partition function and given thresholds of the random variables.
For the given random variables 'E(t)' and 'N(t)' of the ensemble, we define a new non-negative, real-valued exponential variable 'e^(-B(E(t)-M N(t))' with two real-valued parameters 'B' ('=1/kT') and the chemical potential 'M'. 
In the case of quasi-independent and distinguishable systems, Cramer and Chernoff large deviation upper bound 'P*(c)'  on the probability of 'e^(-B(E(t)-M N(t))' expresses in terms of the grand canonical partition function and the given thresholds on the energies and number of particles in the systems,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where 'B > 0', 'Z(B, M)' and 'Z(g)=(Z(B, M))^(X(t))' are the grand canonical partition functions of a single system and the ensemble respectively.
The symbol 'E' in the upper line of equation 6 denotes the mathematical expectation. 
The natural logarithm on both sides of 6, and then division on both sides by 'X(t)', supply
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.  
In equation 9, the limit X(t) to infinity exists. We know that the grand canonical entropy is proportional to the natural logarithm of the probability function 'P*(c)'. 
Equations 7 and 8 give the grand canonical entropies of the ensemble and single distinguishable system respectively, 'S*(c)=k*log*P*(c)=X(t)*[B*E- B*MN + log*Z(B,M)]' and 'S(E, N) =S*(c)/X(t) = k*[B*E+A*N + log*Z(B, A)]', where 'A = -B*M'. The Cramer-Chernoff  large deviation rate function for a single distinguishable system is 'I(E, N) =[-B*E-A*N- log*Z(B, A)] = [(B*G-E)- A*N] ', where the function 'G(B,A)=-(B^(-1))*log*Z(B,A)' is the Gibbs free energy. The rate function 'I(E, N)' shows duality with the Massieu potential function or Planck's characteristic function 'P(B,A)' '(= -B*G =log*Z(B,A)' through the Legendre-Fenchel transform 'log*Z(B, A) =[-B*E-A*N- I(E, N)]'. The rate function the grand canonical ensemble is written as 'I(N)= X(t)*I(E, N)'. We observe that the The Cramer-Chernoff large deviation rate function 'I(c)' or 'I1(E, N)' is identical to the Gibbs index of probability 'N'.  


%Quasi-Independent and Indistinguishable Systems
In the case of quasi-independent and indistinguishable systems, we put the correct form of the grand canonical partition function of the ensemble 'e^(-B*E(t)-M*N(t))/X(t)!' into equation 6 and then follow the steps of calculations of equations 7, and 8. In this case, the Crammer-Chernoff upper bound 'P*(c)' and its natural logarithm, and grand canonical entropy and rate functions are written as
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.
From equation 10, we get the total grand canonical entropy of the ensemble 'S*(c)= k*log*P*(c) = X(t)*S(1c),', where 'S(E, N)=k*[B*E+A*N +log*(eZ/X(t))]' is the entropy of a single indistinguishable system. The Cramer-Chernoff large deviation function for a single indistinguishable system is 'I(E, N)=-k*[B*E+A*N +log*(eZ/X(t))]'.  

%Statistical Equilibrium Condition for the Open Systems
The method of Lagrange's undetermined multipliers subject to restrictive conditions gives the most probable set of the systems 'X(i, N)' for each 'i' at the statistical equilibrium. The entropy or the logarithmic probability function attains the maximum value at the statistical equilibrium. In equations 4 and 8, the entropies $ 'S(b)' and S*(c) are functions of 'X(i,N)'. At the statistical equilibrium, the differentials of logarithmic functions 'dP(b)' and 'dP*(c)', or equivalently the differentials of entropies 'dS(b)' and 'dS*(c)', subject to the variations of the three constraints X=0, Y=0, and Z=0, vanish. 
Following the method of Lagrange's undetermined multipliers, we equate the total variations 'd' of equations 3 and 7 with respect to 'X(i, N)' to zero 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.
where, 'e^(B*G)=1/Z' ,. For the equal values of 'W(N)', we get the probability of finding a distinguishable system in a state with energy 'E(i)' and number of particles 'N(i)', 'X(i,N)/X(t) = e^(- B*E(i)-M*N(i))/Z(B,A)'. By utilizing the total variations of equations 5 and 10, we can obtain a similar expression as that of equation 12, for the probability of finding an indistinguishable system. However, the differences in the Boltzmann-Sanov and grand canonical entropies for indistinguishable and distinguishable cases are functions of 'X(t)'. 

The substitution of 'X(i, N)' from equation 13 into three constraints equation 2 furnishes the expressions for the grand partition function, mean energy, and mean number of particles per system respectively 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
'log*P*(c)[.]< X(t)*[B*E- B*MN + log*Z(B,M)]'.
Using the expressions of 'E*' and 'N*' from 13 in equation 7, the mean grand-canonical entropy per system 'S(c) = S*(c)/X(t)', is,
'S(c) =k[B*E+A*N+ log*Z^(g)]', 
'X=kk[B*E+A*N+ log*Z^(g)]'. 
The recent study of the large deviations shows the connections of entropies or rate function, in terms of equalities and inequalities, with other thermodynamical variables in the reversible and irreversible processes.  
For the reversible processes, the differential of the total Boltzmann-Sanov entropy 'S(b)' shows equality with the differentials of Gibbs free energy and the mean work-done and inequality for the irreversible spatial arrangements of the systems. On the other hand, in the reversible process of the energy and particle with the reservoirs, the differential of total grand canonical entropy establishes equality with differentials of total mean internal energy, total work, and total mean number of particles, 'dS*(c)=B*dQ(c)= B*[dE*(c)+dW(c)-M*dN(c)]'. Both processes of spatial arrangements of the systems and the exchange process of the energy and particle with the reservoirs produce entropy. The entropy productions are zero (always positive) in the reversible (irreversible) processes of spatial arrangements of the open systems and energy and particle exchange with the respective reservoirs. The change in the total entropy of the grand ensemble occurs either due to the production of entropy in the spatial arrangements of open systems inside the ensemble or entropy exchange to or from the heat and particle reservoir. These assertions establish equalities (inequalities) of the total entropy production in the reversible (irreversible) processes of the spatial arrangements and energy-particle exchange 'dS(j)= dS(b)+dS(c)>0'. The upper line of equation 16 shows a strong similarity with the generalized form of the second law of thermodynamics that developed for the black-hole entropy. The middle and lower lines are the equalities (inequalities) of the entropy productions in the reversible (irreversible) diffusion processes that occur interior and exterior of the grand canonical ensemble.

%\sectionLarge Deviations for Spatial and Energy Distributions of Various Systems
Here, we study the large deviations for the distributions of macroscopic variables of various systems such as Planck's and Fermi's ideal linear oscillators, classical and quantum ideal gases, and the magnetic system of particles with spin. Previous studies on these systems utilized the Boltzmann's distribution for the spatial arrangements of members of a system and determined the most probable values using Lagrange's method of undetermined multipliers subject to the restrictive conditions on the total numbers of members and total energy of the system. Moreover, these studies ignored the BCM type probability inequality either for the total internal energy or for both the total number of particles and the total internal energy of the whole ensemble. 

To obtain large deviation results for each of the systems mentioned here, we repeat the following steps: (1) Follow the restrictive conditions and construct the joint spatial distribution for the members of a system and then, by taking the natural logarithm of spatial distribution and using Stirling's approximation for the factorials, obtain Boltzmann-Sanov entropy and rate functions for the macro-state a system and its member. (2) Calculate first the Cramer-Chernoff large deviation probability upper bound either on the total energy or both total numbers of members and the total energy of a system and then use of the natural logarithm of probability function and Stirling's approximation for the factorials provide the entropy and rate functions for the macro-state a system and its member. (3) Establish the statistical equilibrium condition from the differentials of either Boltzmann-Sanov and canonical or grand canonical entropies or the large deviation rate functions by using Lagrange's method of undetermined multipliers and by following the total variation of restrictive conditions on the total energy and total numbers of members of a system. 

% up to here.
%Planck Case: System of the Ideal Linear Oscillators
Planck considered a distribution of the ideal linear oscillators over the infinitesimal region elements of the state-space of the whole system. The notations are similar to those of Planck's book and his research articles. Let '(N=N1+N2+...+N(n)+...)' and '(E=E1+E2+...+E(n)+...)' be the total number of oscillators and the total energy of a system respectively. The subscript 'n' denotes the labeled region elements '(1,2,...,n,....)' of the state-space of a system. The variables 'N(n)' and 'E(n)' are the number of oscillators and their energies in the 'n-th' region respectively. The energy 'E(n)' of the 'N(n)' oscillators with the equal frequency 'f' in the 'n-th' region is 'E(n)=N(n)*(n-1/2)*h*f =  N*w(n)*(n-1/2)h*f', where 'h' is Planck's constant and 'w = Nn/N' is a distribution density. Here, the term '(n-1/2)*h*f' is the arithmetic mean of energies '(n-1)*h*f' and 'n*h*f' of the oscillators in the 'n-th' region. One can also take arithmetic mean over 'n' and 'n+1' region elements; then energy becomes 'E(n)=N(n)*(n+1/2)*h*f'. Moreover, the total energy 'E' of the whole system is the sum of energies of oscillators in all region elements  'E = N*h*f *(n-1/2)*w(n)', where 'w(n) = N(n)/N' is a probability. We can rewrite the total energy as 'E = N*U*', where 'U* = (n-1/2)*w(n)*h*f' is the mean energy per oscillator. 

Following step (1) and the constraints on the total number and total energy of the oscillators, we write large deviations results for the joint spatial distribution of the 'N' quasi-independent linear oscillators over all the region elements
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where 'N(n) > 0', 'w(n)=N(n)/N', '0< w(n)<1', and 'w(n)=1'. From equation 16, the total Boltzmann-Sanov entropy of the system is  'S(bp) = k*log*P(bp) ~ k*[N(n)*log*N - N(n)*log*N(n)]'. Besides, equation 18 gives the entropy of a single ideal oscillator is the mean logarithm of 'w(n)', 'S(bp)= S(bp)/N = -k*[w(n)*log*w(n)]=-k*(<log*w(n)>)'. The Boltzmann-Sanov rate functions for the system and single oscillator are negative of their respective entropies.

Step (2) gives the Cramer-Chernoff large deviation upper bound for the exponential variable of the total energy 'E' of the system. 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
Here 'B>0' and the symbol 'E' in equation 18 denotes the mathematical expectation, and 'Z1(B)=e^(-B*E1)' and 'Z(B)=e^(-B*E)=(e^(-B^E1))^(N)' are the partition functions, respectively, of the single oscillator and the whole system. The equations 19 and 20 supply the expressions, respectively, for the total canonical entropy of the system and the canonical entropy per oscillator 'S*(cp)=k*log*P*(cp) = k *[B*N*U+ N*log*Z1] ' and 'S(cp) = S*(cp)/N=k*[B*N*U+ N*log*Z1]'. For the system and an oscillator, the Cramer-Chernoff large deviation rate functions are 'I=-S/k' and 'I1=S1/k'.

At the statistical equilibrium, the 'd' variations of the entropies with respect to 'N(n)' vanish i.e. 'dS(bp) =0' and 'dS*(cp) =0'. We follow step (3) and get the statistical equilibrium condition for the most probable set of Planck's linear oscillators,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
where the partition function of an oscillator, 'Z1(B)=e^(-B*(n-1/2)*h*N)', is obtained by putting 21 in the condition 'N=N(n)'. Therefore, from equation 21, 'w(n)=e^(-B*(n-1/2)*h*N)' is the probability of finding exactly 'N(n)' oscillators in the 'n-th' region element. To obtain equation 21, we can also consider 'd' variations of equations 17 and 20 with respect to 'w(n)' and follow Lagrange's method of undetermined multipliers.
Using equation 21, the mean energy, 'U*' and mean entropy per oscillator 'S(cp)'  are written, respectively, as
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 

Planck defined a large positive number, the integer 'R' that measures the energy of the system of oscillators, 'R= (E/h*f) -(N/2)=(n-1)*N(n)'. Therefore, by step (1), for a given energy of the system, the joint spatial distribution of 'N' oscillators or the total number of distinct ways of assigning 'R' quanta to 'N' oscillators is
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
Follow step (2) and the Cramer-Chernoff upper bound of the total energy of the system of oscillators is  
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where we have put 'N*U=Rh*ft. The term 'Z1(B)' is the partition function of a single oscillator. Planck replaced the total energy 'E= N*U' of a system of 'N' oscillators with the discrete energy packets of large positive number 'R' (quanta) with finite equal quantity 'h*N', i.e. X=Y/N. Thus, 'E/N=U/N', where 'hu/2' is the zero-point energy.
By considering step (3), for the statistical equilibrium condition, the variations 'dR' of both sides of equations 24 and 26 vanish. 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
The mean energy per oscillator 'E/N' 
E(n)/N=(X*R*N+X)*h*N.

%Bose Case: System of Light Quanta
Let us consider Bose's famous work on the statistics of light quanta. Bose obtained the probability distribution of the light quanta that lie into the various cells of the phase-space of the whole system. Moreover, he reproduced Planck's results of the total entropy of the thermodynamic state and total energy density of the system of the light quanta. We apply steps (1) to (3) sequentially and obtain the large deviations for the distributions of the number of the light quanta and their energies.  The chemical potential 'm' is zero for a system of the light quanta. Here, we follow similar notations found in Bose's work.

Let 'As=Ps,r' be the total number of labeled cells '(Ps0,Ps1,....,P(s,r),...)' in the 's-th' infinitesimal frequency interval 'df'. The index 'r' indicates the number of light quanta in the cells of 'df' . The total number of light quanta and their total energy in the cells of 'df' are 'N(s)=P(s,r)' and 'E(s)=Ps*r*h*fs'  respectively.  These quantities per cell are written as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'
where 'w(r) =Ps,r/As' is a probability, and 'b*' and 'U*(sb)' are, respectively, the mean number of light quanta and their mean energy per cell of 'df'.
Step (1) provides the results for the joint distribution of the cells containing the various number of light quanta in 'df'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'. 
The mean energy per oscillator 'E/N' 
E(n)/N=(X*R*N+X)*h*N.
The distribution over all infinitesimal frequency intervals is the product of distributions, 'P(bb)=W(bb)'. From, 31 and 32, we write the total Boltzmann-Sanov entropy 'S(bb)', and entropy per cell 'S(bb)/As' respectively.
'S(bb) = k *log*W(bb) ~ k *log*(As/P(s,r))', 
S(bb) = k *log*W(bb) ~ k *log*(As/P(s,r))'. 
Moreover, the total entropy of the system over all infinitesimal frequency intervals is 'S(bb) =S(bb)'. The Boltzmann-Sanov rate function are 'I(bb) =-S(bb)' and 'I1(bb) =-S1(bb)'
Considering step (2), for 'B>0, we have expressions for the Cramer-Chernoff large deviation upper bound on the probability of the total energy 'E(s)' of the light quanta, the natural logarithm of probability function, the canonical entropy and Cramer-Chernoff rate function in the interval 'df'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
 'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))',
where '(Z(1,b))^(As)' is the partition function over all 'As' cells. The chemical potential 'M' is zero for the system of the light quanta. The distribution over all infinitesimal frequency intervals is 'P*(c)b=W(bb)'  
Equations 34 and 36 provide the expressions for the total canonical entropy 'S(sb)' and entropy per cell 'S(sb)/As' respectively.
'S(cb)= k *log*W(cb) = [k*B*r*fs + k*r*log*Z(1,b)]', 
'S(cb)= k *log*W(cb) = [k*B*r*fs + k*r*log*Z(1,b)]'. 
Following step (3), the equilibrium condition  is obtained by equating the deviations 'd' on both sides of equations 31 and 35 either with respect to 'ps,r' or with respect to 'w(s,r)' to zero. Here we equate 'dP(s,r)' to zero,
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))', 
where the partition function 'Z(1,b)(B)= e^(-B*r*h*fs)= (1-e^(-B*h*fs))^(-1)' is obtained from the condition 'r=0*P(s,r)= As'. The lower line of equation 38 gives the probability of exactly 'r' number of light quanta that lie in the cells of the interval 'df'. 
Using equation 38, the mean number of light quanta per cell in 'df'  is 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
This is identical with Planck's result (See equation 28).
Moreover, 'N*b=bs= e^(B*h*fs -1)' is the total mean occupancy number of the system of light quanta. 
Using equation 38, the total energy 'E(s)' and energy of the light quanta  per cell in 'df' are obtained, respectively, as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The energy of the whole system of light quanta over all the frequency intervals is 'E(b)=E(s)=B(s)', . 
The mean Gibbs canonical entropy in 'df' at the equilibrium ,is, 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0', 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
where in the second line of equation 41, we have put 'U*(sb)' from equation 40 and logarithm of 'Z(1,b)'. Moreover, the mean Gibbs canonical entropy per cell ,in 'df' from the last line of equation 41 is 
X*S(cb)*As = X*B*h*fs*e^(-B*h*fs-1*log*(1- e^(-B*h*fs)).
Equation 43 is identical to equation 23.
The entropy of the whole system of light quanta over all the frequency intervals is 'S(cb) =M*S(cb)'. 

%Fermi Case: System of Simple Oscillators
Schroedinger studied a simple system of the Fermi oscillators with zero chemical potential. Here the notations are identical to those of Bose's case. The Pauli exclusion principle restricts the number of oscillators (particles) per cell i.e. either  'r=0' or 'r=1' in each cell. The restrictive conditions are defined on the total number of cells 'As', total number of Fermi oscillators 'N(f)' and their energies 'E(f)' in the 's-th' interval, 'As = p(s)', 'N(s)=r*p(s)' and 'E(s)=r*e*p(s)', where 'e' is the energy of a single Fermi oscillator.

Step (1) gives us the joint spatial distribution 'W(bf)' of cells that filled with the oscillators, the total Boltzmann-Sanov entropy 'S(bf)' of the system, and entropy per cell 'S(bf)/As'. 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.'
The last line of equation 44 can be rewritten as 'k*log*W/A=S/A=k<log(w)> '.
We have the total spatial distribution for all the intervals 'P(bf)= W(bf)' and 'S(bf)=S(bf)'.
We consider step (2) and obtain the Cramer-Chernoff's large deviation bound, logarithmic probability function, canonical entropy for the total energy distribution of system of Fermi's oscillators 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
where 'B>0' and 'Z(1,f)=e^(-r*B*E)= (1+e^(-B*E))' is the partition function of a single Fermi oscillator respectively. For the whole system and all the intervals, we get 'P*(cf)=W(cf)' and 'S(cf)= S(cf)'. 
The use of step (3) provides the equilibrium condition for a system of the Fermi oscillators i.e. the most probable values of the oscillators. Equate the 'd' variations of the second line of equation 43 and the third line of equation 44 to zero.  
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0.' 
The lower line of equation 45 defines the probability of finding the Fermi oscillator in the cells of the 's' interval. Using this definition of the probability, equation 47, the mean occupation number of the oscillators per cell 'Sf' is given as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The total occupancy number is 'N*(f)=e^(B*E+1)'. 
Using equation 47, the total energy 'ESf' of oscillators and mean energy per cell and mean energy per cell 'U(sf)f' in the 's-th' interval are written as 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'. 
Putting equation 47 in the mean entropy of oscillators and the mean entropy of oscillators per cell in the 's-th' interval, we get 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0' 
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The total entropy of the system of the Fermi oscillators is 'Sf =N*S(cf)'.  

%Classical and Quantum Ideal Gases
In the previous sections, we have considered the systems of Planck and Fermi ideal linear oscillators, and light quanta with zero chemical potential. Here, we focus on the large deviations study for the distributions of the non-relativistic classical and quantum ideal gases with nonzero chemical potentials. The particles of the ideal gases obey three different types of statistics: (i) Maxwell-Boltzmann (MB) (ii) Bose-Einstein (BE), and (iii) Fermi-Dirac (FD). 
Due to weak interactions between the particles, they are assumed quasi-independent, and thus, the probabilities of macroscopic variables of the particles do not affect each other. Thus the problem of studying the statistics of macroscopic variables of the whole ideal gas reduces to that of studying the statistics of a single particle. Particles of the MB ideal gas are distinguishable and have no restrictions on occupancy in a single state. Bose-Einstein (BE) statistics allows any number of identical and indistinguishable particles (bosons) with integer spin in a single state. In the Fermi-Dirac ideal gas, a single state can not accommodate simultaneously more than one identical and indistinguishable particle (fermion) with half-integral spin because of the restriction of the Pauli exclusion principle. 
Quantum mechanically, the solution for the statistics of an ideal gas is to find the number of symmetric (antisymmetric) eigenfunctions for a boson (fermion) state. Let 'G(j)', 'N(j)', and 'E(j)' be the number of states, number of particles, and their energies in the 'j'-th group. The aggregate of the number of particles '(N(j), j=1,2,...)' into the states of the independent labeled groups 'j=1,2,...' defines the macroscopic state of the whole ideal gas. The total number of particles and total energy of the ideal gas are written as 'N(j)= Nt' and 'N(j)*E(j) = Et'. 

Our first aim is to find the distribution of the 'N(j)' particles that lie into the 'G(j)' states in the 'j'-th group and then in succession construct a distribution for all the independent groups of states. This is equivalent to finding the statistical weight i.e. the number of distinct ways 'G(j)' of distributing 'N(j)' particles over a state in the 'j-th' group. The total statistical weight for all the independent groups of the identical particles is the product of 'G(j)', i.e 'Pb(ig)^(G(j))'.  

Following step (1), the total statistical weights or joint spatial distributions of the particles of the three different types of ideal gases, satisfying the constraints on the total numbers of particles and total energy of the ideal gas, are written as  
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0',
'X*log*P(b)(.) ~ X(i,N)*log*(W(N)/X(i,N))=0'.
The total entropy of an ideal gas is proportional to the natural logarithm of the total statistical weight i.e. 'S(g) ~ k*log*P(ig)= k**log*G(j)'. 
'S(g) ~ k*log*P(ig)= k**log*G(j)',
'S(g) ~ k*log*P(ig)= k**log*G(j)',  
'S(g) ~ k*log*P(ig)= k**log*G(j)'.  
The use of step (2) gives us the Cramer-Chernoff large deviation upper bound on the probability of the variable 'e^(-B*E(t)-M*N(t))', the grand canonical entropy, and the Cramer-Chernoff rate function. 
'P*(c)< e^(-B*E(t)-M*N(t))',
'P*(c)< e^(-B*E(t)-M*N(t))', 
'P*(c)< e^(-B*E(t)-M*N(t))'.
where 'Zg(B,M)' is a grand partition function of whole ideal gas 
and 'A= -B*M'.  We put 'N(t) =N(j)' and 'N(t)U = N(j) E(j) ', and the logarithms of the grand partition functions for the MB, BE, and FD ideal gases in equation 53.
'log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',
'log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'.
We know that the grand canonical entropy for a macroscopic state of an ideal gas is proportional to the natural logarithm of a probability distribution, 'S*(ig) ~k*log*P*(ig); thus, 'S*(ig)= k*log*P*(ig) = S(ig)'. 
Consider step (3), the variations 'dN(j)' on both sides of the set of equations 51 and 54 provide the statistical equilibrium conditions for the set of most probable or mean values of the particles in the three different types of ideal gases.
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',  
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'. 
we get the mean occupation number of the particles in each of the state of 'j-th' group.
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',  
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'. 
The total mean occupancy number of the particles in an ideal gas is 'N=N*(j)'. 

%Magnetic System: Particles with Spins
The absolute temperature 'T' or the parameter 'B=1/kT' is nonnegative, i.e. 'T > 0' or 'B > 0', for for the closed or open normal thermodynamical system.  The internal energy of a normal system varies from zero (0) or a certain least attainable value, say E(+0) to the infinity ('I').
Here we follow steps (1) to (3) and study the large deviations for the distributions of numbers of particles and the total energy of a magnetic system. The internal energy of a magnetic system has both the lower 'Em,+0' and upper 'E-0' bounds, respectively,  for the temperatures 'T tends to +0' and 'T tends to -0'. 

Consider a magnetic system of 'N' weakly interacting quasi-independent particles with a spin '1/2'. This magnetic system is placed in the external magnetic field 'H'; thus, each of the particles has two orientations with a magnetic moment either '+M' parallel to or '-M' antiparallel to the field 'H'. Moreover, the corresponding non-degenerate energies are '+e=+u*H' and  '-e=-u*H'. 
The total number of particles 'N' and the total internal energy 'E' of a system are written as 'N=N++N-' and 'E=(N+-N-)M*H = M*E' respectively, where 'N+' and 'N-' are, respectively, the '+' spin and '-' spin particles, and 'M=N+-N-' is the magnetization. The numbers N+' and 'N-' are expressed in terms of 'M' and 'E' as follows 'N+ = (N+M)/2 = (N*E+E)/2*E ' and 'N- = (N-M)/2 = (N*E-E)/2*E'.    

%For the cases of normal closed or open systems, the temperature 'T' or 'B=1/kT' is nonnegative i.e. 'T > 0' or 'B > 0'. The internal energy of the normal systems or an ensemble varies from '0' (or a certain least attainable value, say 'E+') to 'I'. For the positive attainable temperature 'T > ' or 'B > 0', the internal energy 'E' lie in the interval '(E0, E+] ', where 'E+'  is the maximum value for maximum temperature 'T to infinity ' or 'B tends to +0'. As the temperature 'T tends +0 ' or to least value, then the internal of a system shifts to 'E0', and entropy attains its minimum value. This is the case of the third law of thermodynamics.  The magnetic system of particles with spins is in completely different thermodynamical states for the positive 'T > 0' ('B > 0') and negative 'T < 0' ('B < 0') temperatures. Moreover, at these temperatures, the entropy of the system attains the minimum value but for two entirely different thermodynamics states. Here we study the large deviations for the distributions of the magnetic system corresponding to both positive and negative temperatures. Let 'N+' and 'N-' be, respectively, '+' spin and '-' spin particles. The total number of particles 'N' and the total energy 'E' of the system are written as 'N=N++N-' and 'E=(N+-N-)M H = ME', where 'M=N+-N-' and '*E=M H' respectively. Therefore, we have This system is always termed a 'two-level system'.

By step (1), the number of ways of the spatial arrangements of the N+' and 'N-'  particles in the energy states '+e' and '-e' the thermodynamic weight 'Pb' of a macroscopic state of a magnetic system takes the final form 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))', 
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))',  
'k*log*P*(ig) < P*(c)< e^(-B*E(t)-M*N(t))'. 

In the last line of Eq.58, 'w- = X*N/N' and 'w+=X*N/N' are the probabilities. The Boltzmann-Sanov type entropy ' S(mb)' is Boltzmann constant times the natural logarithm of '*log*P(mb)' i.e. 'S(mb)= k *log*P(mb)'. By putting the values of 'N-' and 'N+' in equation 58, we have the expressions for the total Boltzmann-Sanov type entropy of a system and entropy per particle
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N', 
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N'.

From equation 59, the temperature 'T' of the system is defined as '1/T = dS/dE=(k/*E)*log[(N*E-E)/(N*E+E)]' or '1/T=(k/*E)*log(N+/N-)'. This temperature is either positive or negative according to whether 'N*e < E' or 'N*e > E' 
The parameter 'T* =-1/T' covers the entire range of temperature from '+infinity' to '-infinity' including zero. Table 1 shows the values of 'T', internal energy 'E', and entropy 'S' of a system at various temperatures. The magnetic system is in a completely different thermodynamical states for the positive 'T > 0' ('B > 0') and negative 'T < 0' ('B < 0') temperatures. Moreover, at these temperatures, the entropy of a  system attains the minimum value, but for the entirely different thermodynamical states. In the case of positive temperature, the population in the higher energy state is small 'N(-) <N(+)', whereas for the negative temperature the population is large 'N(-) >N(+)'.
In the experiment on the LiF crystal, by reversing the magnetic field, the thermodynamic equilibrium with the population 'N(-) >N(+)' in the maximum energy state was achieved successfully for the negative temperature. 

We now calculate the Crammer Chernoff upper bound on the probability inequality of the total internal energy 'E' of a system that exceeds to certain threshold 'Nu', where u is the energy per particle. Since the magnetic system exhibits different behavior for both positive and temperature, therefore the maximums of the Crammer Chernoff rate functions are achieved for the intervals of positive and negative temperature with the corresponding ranges of the total internal energies. Therefore we need two probability inequalities for the two intervals of positive and negative temperature. In this case, the population, number of particles, in the maximum energy state is larger than the minimum energy state.

(i) For a  strictly positive temperature 'T >0' ('T* < 0') and corresponding range of the total internal energy of the system, 'Em,+0< E < N*u', we define the probability inequality of the total internal energy and the given threshold 'P*(c)+(E < N*u)=P*(c)+(-E > -N*u)=P*(c)+(-B*E > -B N*u)', where 'B > 0'. (ii)In the case of the negative temperature 'T < 0' ('T*> 0')  and respective range of the total internal energy of a system 'Nu < E < E-0', we get another probability inequality of the total internal energy and the given threshold, 'P*(c)-(E > N*u)=P*(c)-(-B*E > -B*N*u)', where 'B < 0'. Then in the both regimes of positive and negative temperatures of the magnetic system, following step (1), the Cramer-Chernoff large deviation upper bounds and their natural logarithms, canonical entropies and rate functions are written as
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N', 
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N'.
Here the partition function of the whole system is the product of partition functions of the quasi-independent weakly interacting particles. In addition, the Helmholtz free energy of the system is 'A= -N*k*T*log*Z1 = -N*k*T*log(2*cosh(B*E))'. 

Consider step (3) and obtain the statistical equilibrium condition by equating the variations 'd' on sides of the equations 59 and 61 with respect to 'N-' and 'N+'  to zero.
S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N', 
'S(mb) ~ - k *[N- log*X*N-N+N+log*X*N+N'.
The upper and lower lines of equation 62 define the probabilities of finding a single particle of the magnetic system, respectively, in the states 'E+ =M*H' and 'E-=-M*H'. 
The mean energies of a particle and the system are given as 'U* = -d*log(Z1)/dB = -*E*tanh(B*E)' and 'E= M*E= (N+-E-)*E = - N*E*tanh(B*E)=N*U' respectively. 
Moreover, the mean entropies of the system and per particle are, respectively, obtained as 'S(cm) = B*N*U*+N*log*Z(1) = N*k*[-B*E*tanh(B*E)+log(2*cosh(B*E)]' and 'S(mc)= S(cm)/N*k = -B*E*tanh(B*E+log(2*cosh(B*E))'.



%The thermodynamic states of the system at temperatures 'T tends to +_infinity ' are identical. For these temperatures, the internal energy reaches to the mean values 'E +_ infinity' and the entropy attains the maximums 'Sm,+_infinity= N*k*log2'.The parameter 'T* =-1/T' captures all ranges from positive to negative temperatures. 

%For the cases of closed or open normal thermodynamical systems, the temperature $T$ or $\beta=1/kT$ is nonnegative i.e. $T \geq 0$ or $\beta \geq 0$ \cite{LandauV5,Haar95,Schroedinger13,Pathria11,Greiner95}. The internal energy of the normal systems or an ensemble varies from $0$ (or a certain least attainable value, say $E_{+0}$) to $\infty$ \cite{LandauV5,Haar95,Schroedinger13,Pathria11,Greiner95}.  Here we study the large deviations for the distributions of the magnetic system corresponding to both positive and negative temperatures.  The magnetic system of particles with spins is in completely different thermodynamical states for the positive $T \geq 0$ ($\beta \geq 0$) and negative $T \leq 0$ ($\beta \leq 0$) temperatures \cite{Ramsey56,Purcell51}. The internal energy of a magnetic system has lower $\mathsf{E}_{min,+0}$ and upper $\mathsf{E}_{max,-0}$ bounds, respectively, as $T \to +0$ and $T \to -0$ \cite{Ramsey56,Purcell51}. Moreover, at these temperatures, the entropy of the system attains the minimum value but for two entirely different thermodynamics states \cite{Ramsey56,Purcell51}.


\sectionDiscussions and Summary

\bibliographyGrandRef

\enddocument
%
% ****** End of file apstemplate.tex ******


